Rotation Matters: Generalized Monocular 3D Object Detection for Various Camera Systems

Research on monocular 3D object detection is being actively studied, and as a result, performance has been steadily improving. However, 3D object detection performance is significantly reduced when applied to a camera system different from the system used to capture the training datasets. For example, a 3D detector trained on datasets from a passenger car mostly fails to regress accurate 3D bounding boxes for a camera mounted on a bus. In this paper, we conduct extensive experiments to analyze the factors that cause performance degradation. We find that changing the camera pose, especially camera orientation, relative to the road plane caused performance degradation. In addition, we propose a generalized 3D object detection method that can be universally applied to various camera systems. We newly design a compensation module that corrects the estimated 3D bounding box location and heading direction. The proposed module can be applied to most of the recent 3D object detection networks. It increases AP3D score (KITTI moderate, IoU $> 70\%$) about 6-to-10-times above the baselines without additional training. Both quantitative and qualitative results show the effectiveness of the proposed method.

==> def2.tex <==
%
%
%   def.set
%
%       seungjin@postech.ac.kr
%
%       Last updated:
%       September 19, 2004
%
%       A set of my definitions and new commands
%
%


% math bold for lower cases (a-z)
\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bc}{{\mathbf{c}}}
\newcommand{\bd}{{\mathbf{d}}}
\newcommand{\bolde}{{\mathbf{e}}}
\newcommand{\boldf}{{\mathbf{f}}}
\newcommand{\bg}{{\mathbf{g}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\bi}{{\mathbf{i}}}
\newcommand{\bj}{{\mathbf{j}}}
\newcommand{\bk}{{\mathbf{k}}}
\newcommand{\bl}{{\mathbf{l}}}
\newcommand{\bm}{{\mathbf{m}}}
\newcommand{\bn}{{\mathbf{n}}}
\newcommand{\bo}{{\mathbf{o}}}
\newcommand{\bp}{{\mathbf{p}}}
\newcommand{\bq}{{\mathbf{q}}}
\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bz}{{\mathbf{z}}}





% math bold for upper cases (A-Z)
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}





% calligraphic
\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}
\newcommand{\calbX}{\mbox{\boldmath $\mathcal{X}$}}
\newcommand{\calbY}{\mbox{\boldmath $\mathcal{Y}$}}


\newcommand{\bcalA}{\mbox{\boldmath $\calA$}}
\newcommand{\bcalB}{\mbox{\boldmath $\calB$}}
\newcommand{\bcalC}{\mbox{\boldmath $\calC$}}
\newcommand{\bcalD}{\mbox{\boldmath $\calD$}}
\newcommand{\bcalE}{\mbox{\boldmath $\calE$}}
\newcommand{\bcalF}{\mbox{\boldmath $\calF$}}
\newcommand{\bcalG}{\mbox{\boldmath $\calG$}}
\newcommand{\bcalH}{\mbox{\boldmath $\calH$}}
\newcommand{\bcalI}{\mbox{\boldmath $\calI$}}
\newcommand{\bcalJ}{\mbox{\boldmath $\calJ$}}
\newcommand{\bcalK}{\mbox{\boldmath $\calK$}}
\newcommand{\bcalL}{\mbox{\boldmath $\calL$}}
\newcommand{\bcalM}{\mbox{\boldmath $\calM$}}
\newcommand{\bcalN}{\mbox{\boldmath $\calN$}}
\newcommand{\bcalO}{\mbox{\boldmath $\calO$}}
\newcommand{\bcalP}{\mbox{\boldmath $\calP$}}
\newcommand{\bcalQ}{\mbox{\boldmath $\calQ$}}
\newcommand{\bcalR}{\mbox{\boldmath $\calR$}}
\newcommand{\bcalS}{\mbox{\boldmath $\calS$}}
\newcommand{\bcalT}{\mbox{\boldmath $\calT$}}
\newcommand{\bcalU}{\mbox{\boldmath $\calU$}}
\newcommand{\bcalV}{\mbox{\boldmath $\calV$}}
\newcommand{\bcalW}{\mbox{\boldmath $\calW$}}
\newcommand{\bcalX}{\mbox{\boldmath $\calX$}}
\newcommand{\bcalY}{\mbox{\boldmath $\calY$}}
\newcommand{\bcalZ}{\mbox{\boldmath $\calZ$}}

\newcommand{\sfA}{\mbox{$\mathsf A$}}
\newcommand{\sfB}{\mbox{$\mathsf B$}}
\newcommand{\sfC}{\mbox{$\mathsf C$}}
\newcommand{\sfD}{\mbox{$\mathsf D$}}
\newcommand{\sfE}{\mbox{$\mathsf E$}}
\newcommand{\sfF}{\mbox{$\mathsf F$}}
\newcommand{\sfG}{\mbox{$\mathsf G$}}
\newcommand{\sfH}{\mbox{$\mathsf H$}}
\newcommand{\sfI}{\mbox{$\mathsf I$}}
\newcommand{\sfJ}{\mbox{$\mathsf J$}}
\newcommand{\sfK}{\mbox{$\mathsf K$}}
\newcommand{\sfL}{\mbox{$\mathsf L$}}
\newcommand{\sfM}{\mbox{$\mathsf M$}}
\newcommand{\sfN}{\mbox{$\mathsf N$}}
\newcommand{\sfO}{\mbox{$\mathsf O$}}
\newcommand{\sfP}{\mbox{$\mathsf P$}}
\newcommand{\sfQ}{\mbox{$\mathsf Q$}}
\newcommand{\sfR}{\mbox{$\mathsf R$}}
\newcommand{\sfS}{\mbox{$\mathsf S$}}
\newcommand{\sfT}{\mbox{$\mathsf T$}}
\newcommand{\sfU}{\mbox{$\mathsf U$}}
\newcommand{\sfV}{\mbox{$\mathsf V$}}
\newcommand{\sfW}{\mbox{$\mathsf W$}}
\newcommand{\sfX}{\mbox{$\mathsf X$}}
\newcommand{\sfY}{\mbox{$\mathsf Y$}}
\newcommand{\sfZ}{\mbox{$\mathsf Z$}}





% math bold for lower cases (Greek letters)
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bdelta}{\mbox{\boldmath $\delta$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bvarepsilon}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\boldeta}{\mbox{\boldmath $\eta$}}
\newcommand{\btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bvartheta}{\mbox{\boldmath $\vartheta$}}
\newcommand{\biota}{\mbox{\boldmath $\iota$}}
\newcommand{\bkappa}{\mbox{\boldmath $\kappa$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bnu}{\mbox{\boldmath $\nu$}}
\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bpi}{\mbox{\boldmath $\pi$}}
\newcommand{\bvarpi}{\mbox{\boldmath $\varpi$}}
\newcommand{\brho}{\mbox{\boldmath $\rho$}}
\newcommand{\bvarrho}{\mbox{\boldmath $\varrho$}}
\newcommand{\bsigma}{\mbox{\boldmath $\sigma$}}
\newcommand{\bvarsigma}{\mbox{\boldmath $\varsigma$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\bupsilon}{\mbox{\boldmath $\upsilon$}}
\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bvarphi}{\mbox{\boldmath $\varphi$}}
\newcommand{\bchi}{\mbox{\boldmath $\chi$}}
\newcommand{\bpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\bomega}{\mbox{\boldmath $\omega$}}





% math bold for upper cases (Greek Letters)
\newcommand{\bGamma}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bDelta}{\mbox{\boldmath $\Delta$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\bLambda}{\mbox{\boldmath $\Lambda$}}
\newcommand{\bXi}{\mbox{\boldmath $\Xi$}}
\newcommand{\bPi}{\mbox{\boldmath $\Pi$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bUpsilon}{\mbox{\boldmath $\Upsilon$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bPsi}{\mbox{\boldmath $\Psi$}}
\newcommand{\bOmega}{\mbox{\boldmath $\Omega$}}





% vector notation for lower cases (a-z)
\newcommand{\veca}{{\vec{\ba}}}
\newcommand{\vecb}{{\vec{\bb}}}
\newcommand{\vecc}{{\vec{\bc}}}
\newcommand{\vecd}{{\vec{\bd}}}
\newcommand{\vece}{{\vec{\bolde}}}
\newcommand{\vecf}{{\vec{\boldf}}}
\newcommand{\vecg}{{\vec{\bg}}}
\newcommand{\vech}{{\vec{\bh}}}
\newcommand{\veci}{{\vec{\bi}}}
\newcommand{\vecj}{{\vec{\bj}}}
\newcommand{\veck}{{\vec{\bk}}}
\newcommand{\vecl}{{\vec{\bl}}}
\newcommand{\vecm}{{\vec{\bm}}}
\newcommand{\vecn}{{\vec{\bn}}}
\newcommand{\veco}{{\vec{\bo}}}
\newcommand{\vecp}{{\vec{\bp}}}
\newcommand{\vecq}{{\vec{\bq}}}
\newcommand{\vecr}{{\vec{\br}}}
\newcommand{\vecs}{{\vec{\bs}}}
\newcommand{\vect}{{\vec{\bt}}}
\newcommand{\vecu}{{\vec{\bu}}}
\newcommand{\vecv}{{\vec{\bv}}}
\newcommand{\vecw}{{\vec{\bw}}}
\newcommand{\vecx}{{\vec{\bx}}}
\newcommand{\vecy}{{\vec{\by}}}
\newcommand{\vecz}{{\vec{\bz}}}

\newcommand{\vecxi}{{\vec{\bxi}}}
\newcommand{\vecphi}{{\vec{\bphi}}}
\newcommand{\vecvarphi}{{\vec{\bvarphi}}}
\newcommand{\vecbeta}{{\vec{\bbeta}}}
\newcommand{\vecdelta}{{\vec{\bdelta}}}
\newcommand{\vectheta}{{\vec{\btheta}}}


% set of numbers
\newcommand{\Real}{\mathbb R}
\newcommand{\Complex}{\mathbb C}
\newcommand{\Natural}{\mathbb N}
\newcommand{\Integer}{\mathbb Z}


% color
%\definecolor{orange}{rgb}{1,0.3,0}
%\definecolor{copper}{rgb}{1,.62,.40}


% ets
\newcommand{\bone}{\mbox{\boldmath $1$}}
\newcommand{\bzero}{\mbox{\boldmath $0$}}
\newcommand{\0}{{\bf 0}}

\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\bee}{\begin{eqnarray*}}
\newcommand{\eee}{\end{eqnarray*}}

\newcommand{\matrixb}{\left[ \begin{array}}
\newcommand{\matrixe}{\end{array} \right]}   

\newtheorem{theorem}{{Theorem}}
\newtheorem{lemma}{{Lemma}}
\newtheorem{corollary}{{Corollary}}
\newtheorem{definition}{{Definition}}
\newtheorem{proposition}{{Proposition}}
\newtheorem{remark}{{Remark}}
\newtheorem{example}{{Example}}
%\newtheorem{algorithm}{{Algorithm}}

\newcommand{\argmax}{\operatornamewithlimits{\arg \max}}
\newcommand{\argmin}{\operatornamewithlimits{\arg \min}}

\newcommand{\mean}[1]{\left \langle #1 \right \rangle}
\newcommand{\ave}{\mathbb E}
\newcommand{\E}{\mathbb E}
\newcommand{\empha}[1]{{\color{red} \bf #1}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\incomplete}[1]{\textcolor{red}{#1}}



\def\doublespace{\renewcommand{\baselinestretch}{2}\large\normalsize}
\def\singlespace{\renewcommand{\baselinestretch}{1}\large\normalsize}
\def\onehalfspace{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\def\onequaterspace{\renewcommand{\baselinestretch}{1.3}\large\normalsize}
\def\threequaterspace{\renewcommand{\baselinestretch}{1.7}\large\normalsize}
\def\smallspace{\renewcommand{\baselinestretch}{-.9}\large\normalsize}
\def\tinyspace{\renewcommand{\baselinestretch}{-.7}\large\normalsize}

\newcommand{\tr} { \textrm{tr} }
\newcommand{\re} { \textrm{re} }
\newcommand{\diag} { \textrm{diag} }
\newcommand{\ddiag} { \textrm{ddiag} }
\newcommand{\off} { \textrm{off} }
\newcommand{\vectxt} { \textrm{vec} }

\newcommand{\lla}{\left\langle}
\newcommand{\rra}{\right\rangle}
\newcommand{\llbr}{\left\lbrack}
\newcommand{\rrbr}{\right\rbrack}
\newcommand{\llb}{\left\lbrace}
\newcommand{\rrb}{\right\rbrace}


==> hdbbmghpkppdgpsxjsjpbxswkydbdxrq/1_abstract.tex <==
\begin{abstract}
% Monocular 3D object detection은 현재 자율주행에서 활발히 연구되고 있는 분야이다. 현재 monocular 3D object detection network는 학습한 하나의 카메라 데이터 셋에서 준수한 성능을 보여주고 있다. 하지만 학습하지 않은 다른 환경의 카메라 데이터 셋에서는 성능이 현저히 떨어지는 모습을 보인다.
Research on monocular 3D object detection is being actively studied, and as a result, performance has been steadily improving. 
However, 3D object detection performance is significantly reduced when applied to a camera system different from the system used to capture the training datasets. 
For example, a 3D detector trained on datasets from a passenger car mostly fails to regress accurate 3D bounding boxes for a camera mounted on a bus.
In this paper, we conduct extensive experiments to analyze the factors that cause performance degradation.
We find that changing the camera pose, especially camera orientation, relative to the road plane caused performance degradation.
In addition, we propose a generalized 3D object detection method that can be universally applied to various camera systems. We newly design a compensation module that corrects the estimated 3D bounding box location and heading direction.
The proposed module can be applied to most of the recent 3D object detection networks.
It increases AP3D score (KITTI moderate, IoU $> 70\%$) about 6-to-10-times above the baselines without additional training. 
Both quantitative and qualitative results show the effectiveness of the proposed method. 

%We use an existing 3D detector network 


%we observe that state-of-the-art monocular 3D object detectors 
%However, there is performance drop of the monocular 3D object detection network in other untrained camera that has different camera extrinsic parameters. %However, there is a huge performance gap between trained camera and other untrained camera that has different camera extrinsic parameters. % However, there is performance drop of the monocular 3D object detection network in other untrained camera that has different camera extrinsic parameters. 

%This is because the existing monocular 3D object detection methods parameterize the object 3D heading direction 
%우리 페이퍼에서 여러 외부 환경의 카메라 데이터 셋을 만들고 학습하지 않은 다른 카메라 환경에서 성능이 떨어지는 것을 정성적, 정량적으로 확인하였다. 성능이 떨어지는 원인을 규명하였다. 우리는 추가적인 학습없이 간단한 보정을 통해 학습하지 않은 다른 카메라 환경에서 성능이 떨어지지 않는 방법을 제안한다. 만든 데이터 셋과 실제 데이터 셋을 통해 우리 방법의 유용함을 보여주었다.
% In our work, we generate various datasets with different camera extrinsic parameters. Also, we confirm qualitatively and quantitatively that the performance of existing networks decreases in untrained camera dataset. And, we find out the cause of this performance degradation. We propose a method that prevents the performance from decreasing in other untrained camera settings through simple calibration compensation without additional training. Extensive experiments including real dataset show the effectiveness of our method.

% \dots
% \keywords{Monocular 3D object detection, Generalization}
\end{abstract}

==> hdbbmghpkppdgpsxjsjpbxswkydbdxrq/2_introduction.tex <==
\section{Introduction}

% 1. 3D object detection 필요성, 물체 인식 + 3차원 정보 추정

% 3D object detection은 자율주행기술과 같은 실제 적용 분야에서 중요한 역할을 수행한다. 물체의 3D 정보를 검출하는 것은 머신이 3D real world를 알도록 하며 이러한 정보는 collision avoidance 시스템과 머신의 path planning에 이용된다. object의 3차원 정보는 lidar, radar, camera 등 많은 장비로 얻어질 수 있다. 그 중 단안 카메라 3d object detection은 낮은 연산량과 센서 가격, 그리고 실제 환경에 적용하기에 편리함 덕분에 많은 관심을 받고 있으며 많은 연구가 진행되고 있다.
%%% citation 추가 필요
3D object detection is the task of estimating the 3D position and orientation of multiple objects in a scene.
It plays an important role in various visual perception applications such as autonomous driving systems and robot bin picking.
To detect objects in 3D space, conventional methods use various sensors including single cameras, stereo cameras, LiDAR, RADAR or a fusion of multiple sensors \cite{pang2020clocs,fan2021rangedet,sun2021rsn,meyer2019automotive,meyer2019deep,nabati2021centerfusion}.
In particular, recently, single-camera-based 3D object detection, or so-called monocular 3D object detection~\cite{gu2022homography,zhang2021objects,ma2021delving} has attracted increasing interest because a single camera system is cost-effective, light-weight and easily mountable.

% 2. 최근 Monocular 3DOD 연구 ~cite 포함. 어떤식으로 알고리즘이 작동하는지 대략적으로

% monocular 3D object detection은 물체의 depth를 더 잘 뽑는데에 초점이 맞춰져있다. 최근 연구들에는 2D 바운딩 박스와 3D 바운딩 박스 사이의 regression 관계를 이용해 물체의 3D location을 더 잘 학습하려는 방법들이 있었고(monodle, center-based 3dobject detection) object depth에 추가적인 loss를 주어 학습을 하도록 하는 방법들이 있다. (monoflex, homography loss, monodtr)
%%% citation 추가 필요

Monocular 3D object detection is a highly challenging problem because depth information is typically lacking ~\cite{chen2016monocular}.
Recent methods~\cite{lian2021geometry}, \cite{zhang2021objects}, \cite{ma2021delving} decouple the 3D bounding box regression problem into several progressive sub-tasks such as estimating the object 3D center, 3D bounding box size, and 3D heading direction.
These methods disassemble the elements of the 3D bounding box and impose a regression loss for each parameter. This helps to train the entire network effectively and to analyze the contribution of each component. These works currently achieve state-of-the-art performance. 
However, these methods generally do not apply to camera systems mounted on other vehicles (\textit{e.g.} passenger cars, trucks, and buses) even when the same camera model is used. The camera position and orientation are uniquely set based on the vehicle size and platform.
Changes in camera poses drastically degrade the 3D object detection performance.

% Monocular 3D object detection is focused on learning the depth of an object. Recent works attempt to better learning the 3D location of an object using the 3D regression relationship between the 2D bounding box and the 3D bounding box \cite{ma2021delving}, \cite{yin2021center}, and provide the networks an additional loss that is related to object depth \cite{zhang2021objects}, \cite{gu2022homography}, \cite{huang2022monodtr}.


% 3. 기존 연구들의 한계점 (rotation 변화에 따른 성능 하락) 및 그 이유에 대한 설명 (road plane은 고정이라 가정함.)

% 기존의 연구들은 고정된 한 카메라 시스템에서 좋은 퍼포먼스를 내고 있다. 하지만, 실제 시나리오에서는 카메라가 다양한 차량 및 로봇에 부착되기 때문에 카메라 좌표계 고정되어 있지 않으며 이러한 카메라 세팅에서는 기존의 연구들의 성능이 저하될 수 있다. 실제로 기존의 연구들은 고정된 한 카메라로 학습하기 때문에 road plane이 고정되어 있다고 가정하며 학습 및 추론을 하고 있기 때문에 다양한 카메라 좌표계에서 성능이 하락하게 된다. 카메라 Extrinsic의 변화와 같은 상황에 대한 연구는 현저히 부족하다.

%Previous works have achieved high performance with fixed single camera settings. 



% However, in real world, as the camera is attached to various vehicles and robots, the camera coordinate system is not fixed. In fact, most of existing monocular 3d object detection assume that the road plane is fixed because they learn with one fixed camera, so the performance degradation occurs in various camera settings. Also, research on monocular 3d object detection with various camera settings is significantly lacking.


% 4. 제안한 방법이 무엇인지. 3DBB 결과에 given camera pose로 보정함

% 이번 연구에서, 우리는 Camera Extrinsic의 변화가 Monocular 3D object detection에 미치는 영향에 대해 분석하고, 이를 보정하는 방법에 대해 소개한다. 우리는 기존에 많이 사용되는 KITTI 데이터셋에 geometry를 활용하여 다양한 Camera Parameter의 변화를 의미하는 데이터셋을 생성한다. 데이터 생성에 대한 자세한 이야기는 실험 부분을 참고한다. 이후 생성한 데이터를 통해 기존 3D object detector의 성능하락 원인을 분석한다. 우리는 분석한 내용을 바탕으로 성능 하락을 막기 위해 Camera coordinate를 보상해주는 방법을 제안한다. 기존 3D object detector들은 학습에 사용한 데이터셋의 카메라 좌표계에 과적합 되어있다. 때문에 우리는 학습 데이터에서의 카메라 좌표계와 다른 카메라 좌표계를 알고 있을 때, 두 카메라 좌표계 사이를 보정해줌으로써 다양한 camera 변화에서도 기존 3d object detector가 동작 가능하도록 하였다. 많은 실험들을 통해 우리의 방법이 효율적이라는 것을 증명한다.

In this paper, we investigate the root causes of performance degradation. 
To do so, we synthetically generate various images and their corresponding 3D bounding box labels by changing either rotation or translation or both. 
Through extensive experiments, we observe that state-of-the-art monocular 3D object detectors~\cite{qin2019monogrnet,liu2020smoke,ma2021delving,zhang2021objects} produce about $1\%$ $AP_{3D}$ score (KITTI moderate, IoU $> 70\%$) given images captured from different orientations.
Changing the camera orientation in a roll or pitch axis drastically degrades the 3D object detection performance, while changing the camera position and camera orientation in the yaw axis had little effect.
This is because the 3D object detectors have never been trained to regress the 3D heading direction of objects in roll and pitch angles. 
The methods assume that the camera mounted on the vehicle has a fixed position and orientation with respect to the road plane.
They parameterize the 3D heading direction of the vehicles as a single value for yaw-angle, instead of estimating all rotation parameters (roll, pitch, and yaw).

To tackle this issue, we propose a 3D heading compensation module, which is a simple yet effective algorithm for a generalized solution. 
It corrects the estimated object 3D head direction from conventional 3D object detectors, so additional training datasets and training steps are not required. We only need the relative camera orientation between the camera capturing the training data and the camera for the test data. 
We use the pre-calibrated camera extrinsic obtained in the manufacturing process. Extensive experiments with various datasets and ablation studies demonstrate the effectiveness of our method.
Our contributions can be summarized as follows:


% analyze the effects of variations in camera extrinsic on monocular 3D object detection and introduce how to calibrate this problem. We analyze the causes of performance degradation of existing 3D object detectors. Based on our analysis, we find out that existing 3D object detectors are overfitted to the camera coordinate system of the dataset used for training and the performance degradation of those occurs in the camera coordinate system of the untrained dataset. To deal with this problem, we propose a method to compensate for camera coordination. Recognizing the camera coordinate system in the training data and the other camera coordinate system in the inference, our method utilize calibration between the two camera coordinate systems to rotate heading direction of object. Extensive experiment with various datasets shows effectiveness of our method.

\begin{itemize}
    \item We deeply analyze the individual prediction of the 3D object detector and figure out the factors that lead the performance degradation when the model is applied to other camera systems.
    %observe that camera rotation with respect to the road plane affects 3D object detection.
    \item We propose a generalized 3D object detection method that is trained on a specific camera setup but can be utilized in a variety of camera systems.
    \item The proposed method achieves a 6-to-10 times improvement compared to state-of-the-art methods without additional training. 
\end{itemize}




==> hdbbmghpkppdgpsxjsjpbxswkydbdxrq/3_related_work.tex <==


\begin{figure*}[t]
    \centering
        \includegraphics[width=12cm]{figure/overview/Overview.pdf}
    \vspace{-0.1cm}
    \caption{Overview of the proposed 3D object detection pipeline. We utilize a pretrained 3D object detection network (\textit{e.g.} MonoGRNet~\cite{qin2019monogrnet}, SMOKE~\cite{liu2020smoke}, MonoDLE~\cite{ma2021delving}, and MonoFlex~\cite{zhang2021objects}). The proposed 3D heading compensation module rotate the heading direction of initial estimation in yaw-axis. We use precalibrated camera pose $[\mathbf{R}|\mathbf{t}]$ between a source camera (training set) and a target camera (test set). }
    \vspace{-2mm}
\label{overview}
\end{figure*}


\section{Related Works}

\textbf{Monocular 3D Object Detection} Monocular 3D object detection methods estimate the 3D bounding box from a single RGB image. Estimating 3D information from only 2D information is a challenging problem. Mono3D \cite{chen2016monocular} utilizes the prior knowledge of car shape to estimate the 3D bounding box. DeepMANTA \cite{chabot2017deep} and ROI-10D \cite{manhardt2019roi} uses a 3D CAD model of vehicles and estimates the vehicle 3D bounding box using a robust 2D/3D vehicle part matching.
These methods require expensive amounts of training data including car shapes or 3D CAD models and require heavy computational time.
Another research direction incorporates a 2D detection network with a depth estimation network for monocular 3D object detection \cite{xu2018multi,qin2019monogrnet}. SMOKE \cite{liu2020smoke} predicts 3D object detection by combining 3D projected keypoints with regressed 3D regression parameters in an end-to-end manner. MonoDLE \cite{ma2021delving} estimates a coarse center, then reduces the location error between the 2D box center and the projected 3D box center. MonoFLEX \cite{zhang2021objects} separates the truncated object and the edge of the feature map to minimize the object depth estimation error. 

\textbf{Robust Monocular 3D Estimation to Camera Pose Changes}
Recently, monocular 3D geometry estimation tasks, such as depth estimation~\cite{baradad2020height,zhao2021camera} and 3D object detection~\cite{zhou2021monocular,li2021exploring,lian2021geometry} suffer from generalization issues with camera pose changes. 
Some works \cite{baradad2020height,zhao2021camera} propose generalized monocular depth estimation methods. 
The former predict camera pose and estimate depth in the world coordinates. The latter points out the problem of unbalanced distribution of camera extrinsic in training data, and tackles the issue through geometry-aware data augmentation.

Using monocular 3d object detection, Ego-Net \cite{li2021exploring} estimates the pose of each object relative to the camera pose to improve detection performance. Another work \cite{rangesh2020ground} inputs additional information such as a ground plane database or camera calibration parameters to detect the particular object, and is robustly accurate regardless of the plane. MonoEF \cite{zhou2021monocular} proposes a robust algorithm even with a change in camera extrinsic by fusing a visual odometry method and monocular 3d object detection.
In addition to MonoEF \cite{zhou2021monocular}, several recent methods try to solve the problem of robustness in monocular 3D object detection~\cite{li2021exploring,lian2021geometry}. However, existing methods require additional training of the model using the generated images, so the change is limited, unlike a real environment.

% In this work, we propose a generalized 3D object detection that is applicable to various camera systems without additional training. 
% Our method produces accurate 3D object location and heading direction for different camera settings while avoiding performance degradation in different camera settings. 


% We generate the dataset with various camera extrinsic parameters and find out that monocular 3D object detection degrade depending on the camera poses. Our method avoids the performance degradation of monocular 3D object detection network according to camera pose without additional training.

% 우리는한거 쓰기~~
% 우리는 여러 카메라 환경의 데이터 셋을 만들었고 카메라 포즈에 따라 monocular 3d object detection이 성능이 저하되는 문제를 발견했다. 우리의 방법은 추가적인 학습없이 카메라 포즈에 따른 monocular 3d object detection network의 성능 저하를 막는다 막는다.


==> hdbbmghpkppdgpsxjsjpbxswkydbdxrq/4_method.tex <==
\section{Method}

% 이름후보 및 이전이름
% 이전이름 : camera extrinsic parameters change dataset
% Image generation with different camera extrinsic parameters on KITTI 
% generate new kitti image with different camera extrinsic parameters (camera settings)


%We first introduce the data generation method with different viewpoints to investigate the effect of changing camera setting and results on the 3D object detection task in~\secref{sec:datageneration}. Then, we present the proposed 3D object detection method that is generalized to various camera systems in~\secref{sec:ours}.


% 

%% Image generation with different camera extrinsic parameters on KITTI
%% Generating Images from Different Viewing Directions
\subsection{Image synthesis with different camera poses}
\label{sec:datageneration}
We generate images as if they are captured from different positions and orientations by applying the basic knowledge of multiple view geometry~\cite{hartley2003multiple} on KITTI datasets~\cite{geiger2012we}.
For image synthesis, we need an image, a per-pixel depth map, and camera parameters.
KITTI provides all of them, but the 3D points are sparse so we need additional dense depth map computation.
We estimate a dense depth map using the state-of-the-art stereo matching network, HITNET~\cite{tankovich2021hitnet}. 
Given depth map $\mathbf{D}\in \mathbb{R}^{H\times W}$, and pre-calibrated camera intrinsic $\mathbf{K}$, we generate a new image $\mathbf{I}_{target}\in \mathbb{R}^{H\times W}$ in \figref{Qualitative_result_kitti}-(b-f)  by back-projecting the reference image $\mathbf{I}_{ref}\in \mathbb{R}^{H\times W}$ in \figref{Qualitative_result_kitti}-(a) into 3D world space, then re-project the 3D points into a new image plane with the relative camera pose $[\mathbf{R}|\mathbf{t}]$ as follows:
\begin{equation}
\begin{gathered}
    % \mathbf{x}' = \mathbf{K}[\mathbf{R}|\mathbf{t}]\big((\mathbf{K}^{-1}\mathbf{x})d\big),~d\in \mathbf{d},\\
    \mathbf{I}_{target}(\mathbf{x}) = \mathbf{I}_{ref}(\mathbf{x}'),~\text{where}\\
    \mathbf{x}' = \pi\big(\mathbf{K}[\mathbf{R}|\mathbf{t}]\begin{bmatrix}
\mathbf{X}\\
1
\end{bmatrix}\big),~\mathbf{X} = \big(\mathbf{K}^{-1}\begin{bmatrix}
\mathbf{x}\\
1
\end{bmatrix}\big)\mathbf{D}(\mathbf{x}),\\
\end{gathered}
\end{equation}
where $\mathbf{x}=[x,y]^{\intercal}$ and $\mathbf{X}=[X,Y,Z]^{\intercal}$ are 2D image coordinates and 3D camera coordinates, respectively. The projection function $\pi(\cdot)$ maps 3D points $[a,b,c]$ into 2D pixel coordinates $[a/c,b/c]$.

Since we use the estimated depth from stereo matching, the generated target image $\mathbf{I}_{target}$ contains occlusions and uncertain depth values. We disregard these areas for image warping and fill the holes with a pre-trained image inpainting network~\cite{yu2019free}.
We crop the generated image with $804\times244$ resolution (KITTI original resolution: $1280\times375$) with the same 2D image center to reduce the artifact on the image boundary caused by image warping. 
We generate the target images $\mathbf{I}_{target}$ with the changes in camera translation $\mathbf{t}=[t_x,t_y,t_z]^{\intercal}$ and camera orientation $\mathbf{r}=[r_{pitch}$, $r_{yaw}$, $r_{roll}]$. We consider the KITTI right image to be the generated image translated along the $x$-axis.
We skip generating images with $z$-axis translation because it is widely generalized (\textit{e.g.} the previous and next frames).
We additionally synthesize the images with a combination of both rotation and translation changes.

% As a generated image has holes formed outer boundary, we generate a new image $I_{new}$ in 244$\times$804 resolution. As datasets in different camera extrinsic settings are generated in the size 244$\times$804, we crop the original KITTI left image $I_L$ to the resolution of 244$\times$804 $I_l$ in consideration of the aspect ratio. All new images $I_{new}$ have the same center as original center to keep the viewing field the same. Since there are cases in which objects go out of the screen in the generated image $I_{new}$, if less than 30\% of the objects exist in the image, we redefine its type as DontCare that is excluded from training and evaluation. 


%roll ($r_{roll}$), pitch ($r_{pitch}$), and translation Y + rotation X($r_{pitch}$) change as shown in \figref{gen_images}. 
%Since the monocular 3D object detection network trains yaw, we do not generate rotation Y($r_{yaw}$) dataset. We generate images up to 5 degrees for rotation Z($r_{roll}$) and rotation X($r_{pitch}$). In case of different translation Y, it could be different on rotation X for the camera's field of view. A typical example is the camera attached to the car and truck shown in \figref{overview}. 

%We generate images with rotation Z($r_{roll}$) and rotation X($r_{pitch}$) up to 5 degrees in order to experiment within the possible range. In the case of translation Y data, rotation X($r_{pitch}$) is also added to generate translation Y data, and each data is generated by increasing translation Y by 5cm per degree.

% An image is obtained by projecting points in three dimensional space onto a two dimensional image plane. For example, the KITTI left image $I_L$ is a single 2D image projected onto a plane through a projection matrix $\mathbf{P}$ with intrinsic matrix, rotation matrix $(r_{pitch}=0, r_{yaw}=0, r_{roll}=0)$, translation matrix $\mathbf{t}=[t_x, t_y, t_z]^{\intercal}$. \cite{geiger2012we}  In reality, however, images are obtained from environments with various camera extrinsic parameters such as cameras attached to vehicles or robots, which causes performance degradation of the existing network. Therefore, we generate images with different camera extrinsic parameters using the estimated disparity map to warp the KITTI left image $I_L$ to analyze and solve these problems.


% \begin{figure}[]
%     \centering
%         \includegraphics[width=11cm]{figure/new_image/new_image.JPG}
%     \vspace{-0.1cm}
%     \caption{\textbf{Overview of image generation in various camera extrinsic parameters.} We generate images with different camera extrinsic parameters using the depth map. The depth map is obtained through the estimated disparity map and is used for warping the input KITTI left image $I_L$ into new image $I_{new}$ in different camera extrinsic setting. }
%     \vspace{-2mm}
% \label{new_image}
% \end{figure}

% disparity는 kitti left / right 이미지에서 추출한다. <<<
% The disparity $d$ between left $I_L$ and right $I_R$ KITTI image, with a pair of pixel correspondences $x_l$ in $I_L$ and $x_r$ in $I_R$ as follows:
% \begin{equation}
% \begin{gathered}
%     d = x_l - x_r
%     %\text{d}= \text{$x_l$ - $x_r$}
% \end{gathered}
% \end{equation}

%  left 이미지에 있는 픽셀값 x_l의 depth 값에 관해 depth z와 disparity d는 이러한 관계가  성립한다. <<< 
% Regarding the depth value of the pixel $x_l$ in the left KITTI image $I_L$, the relationship between the disparity $d$ and its corresponding depth $z$ can be formulated as:
% \begin{equation}
% \begin{gathered}
%     d =\frac{f\cdot b}{z}
%     % d = f*b / z
% \end{gathered}
% \label{disparity_depth_equ}
% \end{equation}
% where $f$ and $b$ are the camera focal length, and the baseline of the stereo camera pair, respectively.

%우선 disparity를 구하기 위해, KITTI left right 이미지와 pretrained HITNET 네트워크를 이용해 disparity를 구하였다. Then, 카메라 파라미터들과 disparity와 depth 간의 관계를 통해 depth를 구하였고 left 이미지상 pixel들의 3차원 공간 상의 점들을 구하였다. monocular depth network를 이용해 left 이미지의 depth를 바로 구하는 방법도 존재하지만 stereo 이미지를 이용해 disparity를 구하고 left 이미지의 depth를 구하는 방법이 정확도가 더 높기 때문에 이러한 방법을 사용하였다. <<< 이 부분은 안 쓰는게 낫겠죠?
% First, in order to obtain disparity, we use KITTI left image $I_L$, right images $I_R$ and the pretrained HITNET\cite{tankovich2021hitnet}. Then, we obtain depth through the relationship between camera parameters and disparity as shown Equ \eqref{disparity_depth_equ}. 
% \begin{equation}
% \begin{gathered}
%     s\mathbf{x} = \mathbf{P}\mathbf{X}, \\
%     \mathbf{P} = \mathbf{K}[\mathbf{R}|\mathbf{t}]
%     % d = f*b / z
% \end{gathered}
% \end{equation}

%x2d, y2d는 image 2d coord, x3d, y3d, z3d는 camera 3d coord
%where $\mathbf{x}=[x_{2d}$, $y_{2d}]^{\intercal}$ are 2D image pixels, $\mathbf{X}=[x_{3d}$, $y_{3d}$, $z_{3d}]^{\intercal}$ are object's location in 3D camera coordinates and $s$ is a constant. 
%In here, $z_{3d}$ is same with depth. 
%우리는 the depth map을 이용해서 left image에서 다른 카메라 외부변수를 지닌 이미지로 와핑을 시켰다. (+그림추가) 생성된 이미지에는 hole, occlusion들이 존재하게 되는데 우리는 마스크를 만들어서 이미지 pretrained 임페인팅 네트워크와 interpolation을 이용해 채워주었다. 
%We use the depth map from estimated disparity to warp the left KITTI image $I_L$ to the image $I_{new}$ with different camera extrinsic parameters. 
% As the generated image $I_{new}$ has holes and occlusions, we fill them with a pre-trained image inpainting network\cite{yu2019free} and interpolation.
 %we generate a binary mask $I_{mask}$ of the holes and occlusions, and 

%여러 데이터들을 244 * 804 크기로 생성했기 때문에 aspect ratio를 고려해 original 이미지를 원본 이미지 중심 기준으로 244 * 804 크기로 crop 하여 새로 생성하였다. 새로 만든 244 * 804 크기의 원본 데이터로 모델을 학습시켰으며 학습한 모델을 이용해 생성된 여러 이미지들에 대해 inference하며 실험을 진행하였다. 모델들은 monogrnet / smoke / monodle / monoflex가 이용되었으며 최신 다른 monocular 3d od 모델에도 적용가능하다
% We generate datasets $I_{new}$ with rotation Z($r_{roll}$), rotation X($r_{pitch}$), and translation Y + rotation X($r_{pitch}$) change as shown in \figref{gen_images}. Since the monocular 3D object detection network trains yaw, we do not generate rotation Y($r_{yaw}$) dataset. We generate images up to 5 degrees for rotation Z($r_{roll}$) and rotation X($r_{pitch}$). In case of different translation Y, it could be different on rotation X for the camera's field of view. A typical example is the camera attached to the car and truck shown in \figref{overview}. 

%  우리는 rotation Z , X를 몇도 몇도만큼 데이터를 만들었으며 translation Y 의 경우 cm + pitch 만큼 데이터를 만들었다.
% We generate images with rotation Z($r_{roll}$) and rotation X($r_{pitch}$) up to 5 degrees in order to experiment within the possible range. In the case of translation Y data, rotation X($r_{pitch}$) is also added to generate translation Y data, and each data is generated by increasing translation Y by 5cm per degree.

%warping을 통해 새로운 이미지를 만들어내는 것이기 때문에 외부에 hole가 생길 수 있기 때문에 244 * 804 이미지로 만들어주었다. 우리는 모든 새로운 이미지들의 center는 view를 최대한 동일하게 가져가기 위해 original center와 동일하게 이미지를 생성하였다. 생성된 이미지에서 물체들이 화면 밖으로 나가게 되는 경우가 존재하므로 물체의 30퍼센트 이하만이 이미지에 존재한다면 type을 DontCare로 주어 학습 및 평가할 때 제외하도록 하였다.
% As a generated image has holes formed outer boundary, we generate a new image $I_{new}$ in 244$\times$804 resolution. As datasets in different camera extrinsic settings are generated in the size 244$\times$804, we crop the original KITTI left image $I_L$ to the resolution of 244$\times$804 $I_l$ in consideration of the aspect ratio. All new images $I_{new}$ have the same center as original center to keep the viewing field the same. Since there are cases in which objects go out of the screen in the generated image $I_{new}$, if less than 30\% of the objects exist in the image, we redefine its type as DontCare that is excluded from training and evaluation. 

\begin{figure*}[t]
    \centering
    %\resizebox{\columnwidth}{!}{
    \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}}
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/Roll_before/000010_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/Roll_after/000010_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/transY_before/000010_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/transY_after/000010_3D.pdf}\\
         \rotatebox[origin=l]{90}{MonoDLE} \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/cropped/ori_crop.pdf}&
         \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/transX/000021_exi.pdf}&
         \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/transY/000188_exi.pdf} \\
         \rotatebox[origin=lc]{90}{      Ours} \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/cropped/ori_crop.pdf}&
         \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/transX/000021_ours.pdf}&
         \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/transY/000188_ours.pdf} \\
         (a) Original & (b) $x$-translation & (c) $y$-translation\\
         \rotatebox[origin=l]{90}{MonoDLE} \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/pitch/000093_exi.pdf}& 
         \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/yaw/000067_exi.pdf}& 
         \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/roll/000062_exi.pdf}\\
         \rotatebox[origin=lc]{90}{Ours} \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/pitch/000093_ours.pdf} &
         \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/yaw/000067_ours.pdf} & 
         \includegraphics[width=0.3\linewidth]{figure/3D_results_vis/roll/000062_ours.pdf} \\ 
         (d) $x$-rotation & (e) $y$-rotation & (f) $z$-rotation \\
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/Roll_before/000038_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/Roll_after/000038_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/transY_before/000152_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/transY_after/000152_3D.pdf}\\
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/Roll_before/000049_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/Roll_after/000049_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/transY_before/000095_3D.pdf}&
        %  \includegraphics[width=0.24\linewidth]{figure/3D_results_vis/transY_after/000095_3D.pdf}\\
        % (a) & (b) & (c) & (d) \\
    \end{tabular}%
    %}
    \vspace{-0.1cm}
    \caption{Qualitative results of MonoDLE (Top) and Ours (Bottom). Projected 3D bounding box (green - prediction) and projected 3D object center (red - GT, blue - prediction) are visualized.}
    \vspace{-2mm}
\label{Qualitative_result_kitti}
\end{figure*}


% 섹션 이름 생각
%%% Ours generalized 3D object detection method
\subsection{Our 3D Object Detection Method}
\label{sec:ours}
We use the conventional monocular 3D object detection networks, MonoGRNet \cite{qin2019monogrnet}, SMOKE \cite{liu2020smoke}, MonoDLE \cite{ma2021delving}, MonoFLEX \cite{zhang2021objects} trained with the cropped original KITTI datasets.
These methods predict the projected 3D object center $[x_{2d}, y_{2d}]^{\intercal}$, depth $z_{3d}$, yaw angle $r_{yaw}$, and 3D Bounding Box (BB) size $\mathbf{S}=[h,w,l]$, then the object 3D bounding box is computed by \eqnref{eq:objectcenter} and \eqnref{our_method}.
First, the 3D object center $\mathbf{X}_{c}=[X_{c},Y_{c},Z_{c}]$ is computed as follows:
\begin{equation}
\begin{gathered}
    \mathbf{X}_{c} = \begin{bmatrix}
    {X}_{c} \\
    {Y}_{c} \\
    {Z}_{c}
    \end{bmatrix}=z_{3d}\bigg(\mathbf{K}^{-1}\begin{bmatrix}
    {x}_{2d}\\
    {y}_{2d}\\
    1
    \end{bmatrix}\bigg).
\end{gathered}
\label{eq:objectcenter}
\end{equation}
Then, the final output of the object's 8 corners is the eight corner 3D bounding box $\mathbf{B}_{prev}$ computed as follows:
\begin{equation}
\begin{gathered}
    \mathbf{B}_{prev} = \mathbf{R}_{y}(r_{yaw})\begin{bmatrix}
\pm h/2\\
\pm w/2\\
\pm l/2
\end{bmatrix}+\begin{bmatrix}
X_{c}\\
Y_{c}\\
Z_{c}
\end{bmatrix},
\end{gathered}
\label{prev_method}
\end{equation}
where $h, w$, and $l$ are the height, width and length of the 3D bounding box. They represent the 3D heading direction with the yaw axis instead of all orientations (roll, pitch, yaw-axis), which means the camera-to-road relative camera pose is fixed.  
This is a reasonable assumption because the position and angle of the camera system mounted on a vehicle is fixed in the manufacturing process. 
However, this mild assumption causes a drastic performance drop when the model is applied to other camera systems. 
To improve the generalization performance of the models for various camera systems, we design the 3D heading compensation module as shown in \figref{overview}.
Given the relative camera pose $\mathbf{r}_{r\rightarrow t}=[\hat{r}_{roll}, \hat{r}_{pitch}, \hat{r}_{yaw}]$ between a reference camera (training set) and a target camera (test set), we build the final bounding box $\mathbf{B}_{ours}$ as follows:
\begin{equation}
\begin{gathered}
    \mathbf{B}_{ours} = \mathbf{R}_{3d}\begin{bmatrix}
\pm h/2\\
\pm w/2\\
\pm l/2
\end{bmatrix}+\begin{bmatrix}
X_{c}\\
Y_{c}\\
Z_{c}
\end{bmatrix},~\text{where}\\
\mathbf{R}_{3d}=\mathbf{R}_{z}(\hat{r}_{roll})\mathbf{R}_{y}(r_{yaw})\mathbf{R}_{x}(\hat{r}_{pitch}),\\
\end{gathered}
\label{our_method}
\end{equation}
where $\mathbf{R}_{x}(r)$ is the rotation matrix rotating $r$-degree in the $x$-axis.
We use pre-calibrated roll ($\hat{r}_{roll}$) and pitch ($\hat{r}_{pitch}$) angles while the predicted yaw angle ($r_{yaw}$) is utilized from a network, either MonoGRNet, SMOKE, MonoDLE or MonoFLEX.

% \begin{equation}
% \begin{gathered}
% \end{gathered}
% \label{3D_coord}
% \end{equation}

% \begin{equation}
% \begin{gathered}
%\mathbf{X}^{new}_{C} = \begin{bmatrix}
%{x}^{'}_{3d}, {y}^{'}_{3d}, {z}^{3d}
%\end{bmatrix} .
% \end{gathered}
% \label{new_3D_coord}
% \end{equation}
%%% 먼저, 네트워크가 구한 projected 3D object center를 homography image로 보낸다. (in equ2) 그리고, 네트워크가 구한 해당 pixel의 depth를 통해 카메라 extrinsic 3D상 좌표를 구하고 (in equ2) 기존 카메라와 바뀐 카메라 환경의 rotation 만큼 좌표를 반대로 회전하여 이동시켜 준다. (in equ4) 최종 3D object center는 rotation만큼 좌표를 반대로 이동시켜준 x, y와 네트워크에서 추정한 depth를 z로 최종 3D object center로 보정하여 준다.
% First, we get normalized image points using projected 3D object center obtained by network in \eqnref{normalized_img_coord}. And, we use depth($z_{3d}$) of projected 3D object center obtained by network and get 3D coordinates($X_{3d}$) in \eqnref{3D_coord}. Finally, we move 3D coordinates to new 3D coordinates($X^{'}_{3d}$) by rotating in opposite orientation as much as the rotation of the original camera setting and the different camera setting. 
%%% 마지막 줄까지 써야하는지 의문. (depth는 네트워크에서 추출한거로 그대로 사용) 

% corner




% In the case of KITTI left image $I_L$, the projection matrix is composed of intrinsic matrix $\mathbf{K}$, rotation matrix $\mathbf{R}=\mathbf{I} (r_{pitch}=0, r_{yaw}=0, r_{roll}=0)$, and translation matrix $\mathbf{t}=[t_x, t_y, t_z]^{\intercal}$. However, in the case of various camera extrinsic settings, the rotation matrix and translation matrix are not the same as those of KITTI left dataset. Using the same projection matrix as KITTI left's in other camera extrinsic settings, the object's 3D bounding box is formed without being attached to the ground. In fact, using KITTI right image, 3D bounding box is properly detected when the right projection matrix is used. Therefore, in different extrinsic camera setting, it is appropriate to use the projection matrix with the appropriate rotation and translation values. 

%\begin{figure}[]
%    \centering
    %\resizebox{\columnwidth}{!}{
%    \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}}
%         \includegraphics[width=0.48\linewidth]{figure/appropriate_calib/noncalib/000049_3D.png}&
%         \includegraphics[width=0.48\linewidth]{figure/appropriate_calib/cliab/000049_3D.png} \\
%         \includegraphics[width=0.48\linewidth]{figure/appropriate_calib/noncalib/000178_3D.png}&
%         \includegraphics[width=0.48\linewidth]{figure/appropriate_calib/cliab/000178_3D.png}  \\
%         inappropriate projection matrix & appropriate projection matrix \\
%    \end{tabular}%}
%    \vspace{-0.1cm}
%    \caption{\textbf{Comparison projection matrix.} When using inappropriate projection matrix on the camera extrinsic setting, the 3D bounding box is always formed in a certain direction whether the ground or objects are rotated. On the other hand, when an appropriate projection matrix is used, the 3D bounding box is formed by properly rotating the ground or objects.}
%    \vspace{-2mm}
%\label{appropriate_calib}
%\end{figure}

%monocular 3d object detection 모델은 2d image를 input으로 받고 각 물체들의 3d location center를 추정하게 된다. 기존의 네트워크는 2D정보만을 이용해 3D 카메라 coordinate를 추정할 수 없으므로 KITTI 데이터 셋에 맞는 고정된 카메라 좌표계에 대해 물체의 3D location을 추정한다. 
% The monocular 3d object detection network receives a 2D image as input and estimates the 3D location center of each object, which is camera 3d coordinates. As the existing network cannot estimate the 3D camera coordinates using only 2D information, the 3D location of the object is estimated using the fixed camera settings that fits the KITTI left datset as shown \eqref{existing_method}

% \begin{equation}
% \begin{gathered}
%     X_{2d} = K^{-1} \times \begin{bmatrix}
% x_{2d}\\
% y_{2d}\\
% 1
% \end{bmatrix}, \\
%     X_{3d} = \begin{bmatrix}
% X_{2d} \times z_{3d}
% \end{bmatrix}
% \end{gathered}
% \label{existing_method}
% \end{equation}

% Where, $x_{2d}$, $y_{2d}$ are object 3D center in 2D image, $z_{3d}$ is the estimated depth of an object, and $X_{3d}$ is the 3D center of an object. 

% %하지만 기존의 네트워크들은 고정된 하나의 카메라 좌표계에서 물체의 3d location을 추정해왔기 때문에 다른 카메라 세팅에서는 물체의 3D location을 잘 추정하지 못한다. % 우리는 새로운 알고리즘을 제안한다. 기존의 네트워크가 학습한 카메라와 새로운 카메라 환경 사이의 상대적 관계를 제공하면 네트워크가 새로운 환경에 대해서도 물체의 3d location을 잘 추정할 수 있게 하는. 
% However, since existing networks have estimated the 3D object of an object in single fixed camera system, it is difficult to estimate the 3D location of an object in other camera system. We propose a new algorithm that allows the network to estimate the 3D location of an object in the new camera settings, given the relative relationship between the learned camera and the new camera settings as shown \figref{overview}.

% \begin{equation}
% \begin{gathered}
%     %
%     X^{'}_{3d} = \begin{bmatrix}
% R^T \mid -R^Tt
% \end{bmatrix} \times X_{3d}

% \end{gathered}
% \label{our_method}
% \end{equation}

% Where, $X{'}_{3d}$ is the compensated 3D center of an object, and $\mathbf{R}$, $\mathbf{t}$ are relation between the existing camera and the new camera. 
% % 우리는 기존의 네트워크가 학습한 카메라와 새로운 카메라 환경 사이의 상대적 관계를 제공하면 새로운 환경에서도 각 물체들의 3D 위치를 잘 추정하는 알고리즘을 개발하였다. 

% Using the \eqnref{our_method}, we compensate the 3D location of an object in the yaw-axis using the given $\mathbf{R}$, $\mathbf{t}$ to correct the 3D location of an object estimated by the existing network. Our method proves its effectiveness through extensive experiments.

% 우리는 새로운 알고리즘을 제안한다. 기존의 네트워크가 학습한 카메라와 새로운 카메라 환경 사이의 상대적 관계를 제공하면 네트워크가 새로운 환경에 대해서도 물체의 3d location을 잘 추정할 수 있게 하는. 


% 기존의 네트워크는 KITTI 데이터 셋에 맞는 고정된 카메라 좌표계에 대해 물체의 3D location을 추정한다. 

% 물체의 3D location의 ground truth는 카메라 3D coordinate으로 표현되므로 네트워크가 물체의 3D location을 추정할 때 projection matrix를 이용하게 된다. KITTI dataset의 projection matrix

%하지만 기존의 네트워크들은 고정된 하나의 카메라 좌표계에서 물체의 3d location을 추정해왔기 때문에 다른 카메라 세팅에서는 물체의 3D location을 잘 추정하지 못한다. 우리는 네트워크가 학습한 카메라와 새로운 카메라 환경 사이의 상대적 관계를 제공하면 새로운 환경에서도 각 물체들의 3D 위치를 잘 추정하는 알고리즘을 개발하였다. 
% 지금까지 네트워크들은 고정된 좌표계를 학습했으므로 
% 각 물체 center location의 ground truth는 camera 3d coordinate로 되어 있으므로 네트워크는 
%At this time, the estimated 3D location center of each object is image 3D coordinates $x_2d$, $y_2d$, $z_3d(=depth)$. The ground truth of the object's 3D location center is the camera 3D coordinates, so the monocular 3d object detection network needs to convert the estimated image 3D coordinates into the camera 3D coordinates. 

%변환할 때, 기존의 방법은 projection matrix를 K[R|T] = K[I | T] (tz = 0으로 취급) 라 가정하고 변환한다. (+앞 수식 참고) KITTI left image 데이터 셋에서는 rotation matrix = I이고(pitch, yaw, roll = 0), tz 값이 매우 작기 때문에 이러한 가정은 kitti left image 데이터셋 내에서는 학습할 때와 추정할 때 유효하다. 즉 해당 데이터셋에서는 image 3d coordinate ->(img to rect) camera 3d coordinate ->(rect to img, projection matrix) image 3d coordinate 가 성립한다. 
%The existing method that converts image 3D coordinates to camera 3D coordinates assumes that projection matrix be K$[R\|T]$=K$[I\|T]$ and $t_z$ be zero. In the KITTI left image dataset, the rotation matrix $R=I (pitch=0, yaw=0, roll=0)$, and the $t_z$ value is very small, so this assumption is valid for training and inference in the KITTI left image $I_L$. That is, in KITTI left image dataset, transforming from image 3D coordinates to camera 3D coordinates and then from camera 3D coordinates to image 3D coordinates is the same as the initial image 3D coordinates. 

%하지만 rotation matrix != I이거나 tz가 큰 값과 같은 다양한 카메라 환경에서는 image 3d coordinate 를 camera 3d coordinate 로 변환할 때 기존의 방법을 이용한다면 image 3d coordinate -> camera 3d coordinate -> image 3d coordinate가 성립하지 않는다. 우리는 이러한 문제를 해결하기 위해 새로운 방법으로 이미지 3d coord에서 카메라 3d 좌표로 변환시켜주었다.
%However, in various camera extrinsic setting such as rotation matrix is not I or a large value of $t_z$, transforming from image 3D coordinates to camera 3D coordinates and then from camera 3D coordinates to image 3D coordinates is not the same as the initial image 3D coordinates when using the existing method. To solve this problem, we propose new method that converts image 3D coordinates to camera 3D coordinates.

%where $X_{2d}$ is normalized image coordinates, $x_{2d}, y_{2d}$ are in image pixel, $X_{3d}$ is a camera 3D coordinates.
% 식 4에 따라 우리는 이미지 위의 점을 normalized image 좌표로 변환하고 depth를 통해 카메라 3차원 좌표를 구한다. 여기서 구한 3d 좌표 값은 카메라의 외부 변수 값들이 반영되어 있지 않다. 따라서 우리는 카메라 외부 변수인 rotation, translation matrix를 반영하도록 R|T의 inverse pose인 [$R^T$ $|$ $-R^Tt$]를 곱해 새로운 3d 좌표 값을 구한다.

%According to Equ \eqref{calibration compensation system}, we transform the pixel on the image into normalized image coordinates and obtain the camera 3D coordinates through the depth $z_3d$. Since the obtained camera 3D coordinates does not reflect the extrinsic parameters of the camera, we obtain a new camera 3D coordinates multiplying the inverse pose of $[R|t]$ by $X_{3d}$ to reflect the rotation and translation of camera.

\begin{table*}[t]
\centering
\begin{footnotesize}
\vspace{0.1cm}
\begin{tabular}{c|c|llllll}
\hline
\multirow{2}{*}{Dataset}                                                  & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{$AP_{3D}(IoU=0.7)$}                            & \multicolumn{3}{c}{$AP_{BEV}$}                    \\ \cline{3-8} 
&                         & E             & M            & \multicolumn{1}{c|}{H} & E             & M             & H             \\ \hline
Original                                                                  & MonoGRNet               & 12.2          & 8.12         & 6.94                   & 21.8          & 17.2          & 13.7          \\ \hline
\multirow{2}{*}{Roll}                                                     & MonoGRNet               & $0.74_{(6\%)}$    & $0.54_{(6\%)}$   & $0.37_{(5\%)}$             & $17.2_{(79\%)}$    & $13.7_{(79\%)}$    & $11.9_{(87\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{10.1}_{(82\%)}$    & $\textbf{6.45}_{(79\%)}$   & $\textbf{4.84}_{(70\%)}$             & $\textbf{18.3}_{(84\%)}$    &$\textbf{16.1}_{(94\%)}$    & $\textbf{13.5}_{(99\%)}$    \\ \hline
\multirow{2}{*}{Pitch}                                                    & MonoGRNet               & $1.29_{(11\%)}$    & $0.81_{(10\%)}$   & $0.57_{(8\%)}$             & $22.9_{(104\%)}$    & $18.0_{(104\%)}$    & $14.1_{(103\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{8.15}_{(67\%)}$    & $\textbf{5.89}_{(73\%)}$   & $\textbf{5.12}_{(74\%)}$             & $\textbf{24.1}_{(110\%)}$    & $\textbf{19.7}_{(114\%)}$    & $\textbf{15.9}_{(116\%)}$    \\ \hline
\multirow{2}{*}{Yaw}                                                      & MonoGRNet               & $8.39_{(69\%)}$    & $5.31_{(65\%)}$   & $4.31_{(62\%)}$             & $21.7_{(99\%)}$    & $16.8_{(97\%)}$    & $13.2_{(96\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{9.54}_{(78\%)}$    & $\textbf{6.37}_{(78\%)}$   & $\textbf{5.5}_{(79\%)}$             & $\textbf{22.2}_{(102\%)}$    & $\textbf{16.9}_{(98\%)}$    & $\textbf{13.1}_{(97\%)}$    \\ \hline
\multirow{2}{*}{TransX}                                                   & MonoGRNet               & $10.7_{(88\%)}$          & $7.89_{(97\%)}$          & $6.17_{(89\%)}$                    & $19.0_{(87\%)}$            & $15.5_{(90\%)}$         & $13.1_{(96\%)}$         \\
& \textbf{+Ours}          & $\textbf{10.7}_{(88\%)}$ & $\textbf{7.89}_{(97\%)}$ & $\textbf{6.17}_{(89\%)}$           & $\textbf{19.0}_{(87\%)}$   & $\textbf{15.5}_{(90\%)}$ & $\textbf{13.1}_{(96\%)}$ \\ \hline
\multirow{2}{*}{TransY}                                                   & MonoGRNet               & $11.1_{(91\%)}$           & $7.71_{(95\%)}$          & $6.37_{(92\%)}$                     & $18.1_{(83\%)}$           & $14.2_{(83\%)}$           & $12.8_{(93\%)}$           \\
& \textbf{+Ours}          & $\textbf{11.1}_{(91\%)}$ & $\textbf{7.71}_{(95\%)}$ & $\textbf{6.37}_{(92\%)}$           & $\textbf{18.1}_{(83\%)}$   & $\textbf{14.2}_{(83\%)}$ & $\textbf{12.8}_{(93\%)}$\\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}TransY\\ + Pitch\end{tabular}} & MonoGRNet               & $1.09_{(9\%)}$    & $0.76_{(9\%)}$   & $0.53_{(8\%)}$             & $17.0_{(78\%)}$    & \textbf[$14.7_{(85\%)}$    & $13.1_{(96\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{8.12}_{(67\%)}$    & $\textbf{6.14}_{(79\%)}$   & $\textbf{5.45}_{(78\%)}$             & $\textbf{17.8}_{(81\%)}$    & $\textbf{16.0}_{(93\%)}$    & $\textbf{14.7}_{(107\%)}$    \\ \hline\hline
Original                                                                  & SMOKE               & 16.58          & 9.56         & 9.12                   &  18.5         & 14.3         & 13.9          \\ \hline
\multirow{2}{*}{Roll}                                                     & SMOKE               & $0.88_{(5\%)}$    & $0.61_{(6\%)}$   & $0.50_{(5\%)}$             & $17.3_{(93\%)}$    & $13.9_{(97\%)}$    & $12.6_{(91\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{13.54}_{(81\%)}$    & $\textbf{7.40}_{(77\%)}$   & $\textbf{6.11}_{(67\%)}$           & $\textbf{18.3}_{(99\%)}$    & $\textbf{17.1}_{(119\%)}$    & $\textbf{15.6}_{(108\%)}$    \\ \hline
\multirow{2}{*}{Pitch}                                                    & SMOKE               & $1.54_{(9\%)}$    & $1.01_{(10\%)}$   & $0.76_{(8\%)}$             & $19.2_{(104\%)}$    & $15.4_{(108\%)}$    & $14.0_{(100\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{9.89}_{(60\%)}$    & $\textbf{6.56}_{(69\%)}$   & $\textbf{6.42}_{(70\%)}$             & $\textbf{20.9}_{(113\%)}$    & $\textbf{16.8}_{(118\%)}$    & $\textbf{15.8}_{(114\%)}$    \\ \hline
\multirow{2}{*}{Yaw}                                                      & SMOKE               & $11.7_{(70\%)}$    & $6.34_{(66\%)}$   & $5.26_{(58\%)}$             & $17.2_{(93\%)}$    & $14.1_{(98\%)}$    & $13.4_{(96\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{13.8}_{(83\%)}$    & $\textbf{7.54}_{(79\%)}$   & $\textbf{6.94}_{(76\%)}$             & $\textbf{17.8}_{(96\%)}$    & $\textbf{14.1}_{(98\%)}$    & $\textbf{13.6}_{(98\%)}$    \\ \hline
\multirow{2}{*}{TransX}                                                   & SMOKE                   & $14.1_{(85\%)}$          & $9.56_{(89\%)}$          & $9.12_{(87\%)}$                    & $18.5_{(98\%)}$            & $14.3_{(102\%)}$         & $13.9_{(94\%)}$          \\
& \textbf{+Ours}          & $\textbf{14.1}_{(85\%)}$ & $\textbf{9.56}_{(89\%)}$ & $\textbf{9.12}_{(87\%)}$           & $\textbf{18.5}_{(98\%)}$   & $\textbf{14.3}_{(102\%)}$ & $\textbf{13.9}_{(94\%)}$ \\ \hline
\multirow{2}{*}{TransY}                                                   & SMOKE                   & $14.8_{(89\%)}$          & $9.11_{(95\%)}$          & $8.56_{(87\%)}$                    & $19.0_{(102\%)}$            & $15.4_{(108\%)}$         & $12.8_{(92\%)}$          \\
& \textbf{+Ours}          & $\textbf{14.8}_{(89\%)}$ & $\textbf{9.11}_{(95\%)}$ & $\textbf{8.56}_{(87\%)}$           & $\textbf{19.0}_{(102\%)}$   & $\textbf{15.4}_{(108\%)}$ & $\textbf{12.8}_{(92\%)}$ \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}TransY\\ + Pitch\end{tabular}} & SMOKE               & $1.33_{(8\%)}$    & $0.89_{(9\%)}$   & $0.61_{(7\%)}$             & $17.0_{(92\%)}$    & $13.9_{(97\%)}$    & $12.0_{(86\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{10.4}_{(63\%)}$    & $\textbf{6.44}_{(67\%}$)   & $\textbf{5.64}_{(62\%)}$             & $\textbf{18.1}_{(98\%)}$    & $\textbf{15.0}_{(105\%)}$    & $\textbf{13.7}_{(99\%)}$    \\ \hline\hline
Original                                                                  & MonoDLE               & 13.6          & 11.3         & 9.69                   & 19.7          &  16.1         & 14.7          \\ \hline
\multirow{2}{*}{Roll}                                                     & MonoDLE               & $1.29_{(9\%)}$    & $0.99_{(9\%)}$   & $0.92_{(9\%)}$             & $17.3_{(88\%)}$    & $14.5_{(90\%)}$    & $12.7_{(86\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{11.8}_{(87\%)}$    & $\textbf{9.10}_{(80\%)}$   & $\textbf{7.98}_{(82\%)}$           & $\textbf{18.3}_{(93\%)}$    & $\textbf{16.7}_{(103\%)}$    & $\textbf{15.0}_{(103\%)}$    \\ \hline
\multirow{2}{*}{Pitch}                                                    & MonoDLE               & $1.96_{(14\%)}$    & $1.76_{(16\%)}$   & $1.45_{(15\%)}$             & $20.0_{(102\%)}$    & $14_{(88\%)}$    & $12.8_{(87\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{9.91}_{(73\%)}$    & $\textbf{9.12}_{(81\%)}$   & $\textbf{7.82}_{(81\%)}$             & $\textbf{21.9}_{(111\%)}$    & $\textbf{16.5}_{(102\%)}$    & $\textbf{16.0}_{(109\%)}$    \\ \hline
\multirow{2}{*}{Yaw}                                                      & MonoDLE               & $9.42_{(69\%)}$    & $6.91_{(60\%)}$   & $5.72_{(59\%)}$             & $20.2_{(102\%)}$    & $17.8_{(110\%)}$    & $16.9_{(115\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{10.7}_{(79\%)}$    & $\textbf{9.44}_{(83\%)}$   & $\textbf{7.87}_{(81\%)}$             & $\textbf{21.6}_{(110\%)}$    & $\textbf{18.9}_{(117\%)}$    & $\textbf{17.4}_{(119\%)}$    \\ \hline
\multirow{2}{*}{TransX}                                                   & MonoDLE                 & $13.6_{(96\%)}$          & $10.1_{(89\%)}$          & $8.89_{(92\%)}$                    & $19.4_{(98\%)}$            & $15.6_{(97\%)}$         & $14.5_{(99\%)}$          \\
& \textbf{+Ours}          & $\textbf{13.6}_{(96\%)}$ & $\textbf{10.1}_{(89\%)}$ & $\textbf{8.89}_{(92\%)}$           & $\textbf{19.4}_{(98\%)}$   & $\textbf{15.6}_{(97\%)}$ & $\textbf{14.5}_{(99\%)}$  \\ \hline
\multirow{2}{*}{TransY}                                                   & MonoDLE                 & $13.8_{(101\%)}$          & $10.8_{(96\%)}$          & $8.56_{(88\%)}$                    & $19.2_{(97\%)}$            & $15.4_{(95\%)}$         & $14.4_{(98\%)}$          \\
& \textbf{+Ours}          & $\textbf{13.8}_{(101\%)}$ & $\textbf{10.8}_{(96\%)}$ & $\textbf{8.56}_{(88\%)}$           & $\textbf{19.2}_{(97\%)}$   & $\textbf{15.4}_{(95\%)}$ & $\textbf{14.4}_{(98\%)}$  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}TransY\\ + Pitch\end{tabular}} & MonoDLE               & $1.81_{(13\%)}$    & $1.44_{(13\%)}$   & $1.29_{(13\%)}$             & $17.5_{(89\%)}$    & $15.0_{(93\%)}$    & $12.8_{(88\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{9.89}_{(73\%)}$    & $\textbf{9.13}_{(80\%}$)   & $\textbf{7.21}_{(61\%)}$             & $\textbf{18.5}_{(94\%)}$    & $\textbf{16.4}_{(102\%)}$    & $\textbf{14.9}_{(101\%)}$    \\ \hline\hline
Original                                                                  & MonoFLEX               & 14.2          & 9.94         & 7.09                  & 19.67          & 16.11          & 14.67          \\ \hline
\multirow{2}{*}{Roll}                                                     & MonoFLEX               & $1.13_{(8\%)}$    & $0.87_{(9\%)}$   & $7.09_{(10\%)}$             & $16.8_{(83\%)}$    & $14.1_{(88\%)}$    & $12.0_{(83\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{11.0}_{(77\%)}$    & $\textbf{7.12}_{(71\%)}$   & $\textbf{5.45}_{(77\%)}$           & $\textbf{18.7}_{(93\%)}$    & $\textbf{16.9}_{(106\%)}$    & $\textbf{14.3}_{(97\%)}$    \\ \hline
\multirow{2}{*}{Pitch}                                                    & MonoFLEX               & $2.12_{(15\%)}$    & $1.34_{(13\%)}$   & $0.99_{(14\%)}$             & $21.0_{(104\%)}$    & $13.9_{(87\%)}$    & $12.9_{(90\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{9.89}_{(60\%)}$    & $\textbf{6.56}_{(69\%)}$   & $\textbf{6.42}_{(70\%)}$             & $\textbf{20.9}_{(113\%)}$    & $\textbf{16.8}_{(118\%)}$    & $\textbf{15.8}_{(114\%)}$    \\ \hline
\multirow{2}{*}{Yaw}                                                      & MonoFLEX               & $9.8_{(69\%)}$    & $6.44_{(65\%)}$   & $4.23_{60\%}$             & $20.2_{(103\%)}$    & $15.8_{(98\%)}$    & $13.8_{(94\%)}$    \\ 
& \textbf{+Ours}          & $\textbf{12.1}_{(85\%)}$    & $\textbf{8.12}_{(82\%)}$   & $\textbf{5.41}_{(76\%)}$             & $\textbf{20.8}_{(106\%)}$    & $\textbf{16.7}_{(104\%)}$    & $\textbf{14.8}_{(101\%)}$    \\ \hline
\multirow{2}{*}{TransX}                                                   & MonoFLEX                & $14.1_{(99\%)}$          & $9.51_{(96\%)}$          & $7.49_{(106\%)}$                    & $19.3_{(98\%)}$            & $15.7_{(97\%)}$         & $14.4_{(98\%)}$          \\
& \textbf{+Ours}          & $\textbf{14.1}_{(99\%)}$ & $\textbf{9.51}_{(96\%)}$ & $\textbf{7.49}_{(106\%)}$           & $\textbf{19.3}_{(98\%)}$   & $\textbf{15.7}_{(97\%)}$ & $\textbf{14.4}_{(98\%)}$ \\ \hline
\multirow{2}{*}{TransY}                                                   & MonoFLEX                & $14.8_{(104\%)}$          & $9.11_{(92\%)}$          & $7.56_{(107\%)}$                    & $19.5_{(99\%)}$            & $15.5_{(99\%)}$         & $14.2_{(97\%)}$          \\
& \textbf{+Ours}          & $\textbf{14.8}_{(104\%)}$ & $\textbf{9.11}_{(92\%)}$ & $\textbf{7.56}_{(107\%)}$           & $\textbf{19.5}_{(99\%)}$   & $\textbf{15.9}_{(99\%)}$ & $\textbf{14.2}_{(97\%)}$ \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}TransY\\ + Pitch\end{tabular}} & MonoFLEX               & $1.94_{(14\%)}$    & $1.27_{(12\%)}$   & $1.09_{(15\%)}$             & $18.8_{(93\%)}$    & $12.1_{(76\%)}$    & $11.1_{(76\%)}$    \\ 
& \textbf{$+Ours$}          & $\textbf{9.57}_{(67\%)}$    & $\textbf{8.54}_{(86\%)}$   & $\textbf{5.89}_{(83\%)}$             & $\textbf{19.7}_{(98\%)}$    & $\textbf{13.8}_{(86\%)}$    & $\textbf{12.7}_{(88\%)}$    \\ \hline\hline
\end{tabular}
\caption{\textbf{Part of quantitative 3D detection results.} An example is improvement when degree is 3. Subscript parentheses indicate the percentage of performance compared to the original dataset performance. E, M, H means easy, moderate and hard, respectively.}
\label{Part_3D_results}
\end{footnotesize}
\end{table*}


==> hdbbmghpkppdgpsxjsjpbxswkydbdxrq/5_experiment.tex <==
\section{Experiments}

\begin{figure*}[t]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c@{\hspace{0.1mm}}c@{\hspace{0.1mm}}c@{\hspace{0.1mm}}c@{\hspace{0.1mm}}}
         \includegraphics[width=0.23\linewidth]{figure/new_3D_graph/MonoGRNet.png}&
         \includegraphics[width=0.23\linewidth]{figure/new_3D_graph/SMOKE.png}&
         \includegraphics[width=0.23\linewidth]{figure/new_3D_graph/MonoDLE.png}&
         \includegraphics[width=0.23\linewidth]{figure/new_3D_graph/MonoFLEX.png} \\
         (a) MonoGRNet & (b) SMOKE & (c) MonoDLE & (d) MonoFLEX
    \end{tabular}
    }
    \vspace{-0.1cm}
    \caption{3D object detection results. The $x$-axis is the rotation angle and the $y$-axis is the performance drop ratio ($\%$) compared to the $AP_{3D}$ (KITTI moderate, IoU=0.7) result of the original image.}
    \vspace{-2mm}
\label{3D_results_graph}
\end{figure*}




% \begin{figure*}[t]
% \centering
% \footnotesize
% \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}}
%         \includegraphics[width=0.3\linewidth]{figure/gen_all/original.pdf}&
%         \includegraphics[width=0.3\linewidth]{figure/gen_all/transX.pdf}&
%         \includegraphics[width=0.3\linewidth]{figure/gen_all/transY.pdf}\\
%         (a) KITTI original image (left) & (b) Image translated in \textit{x}-axis ($t_{x}$) & (c) Image translated in \textit{y}-axis ($t_{y}$) \\
%         \includegraphics[width=0.3\linewidth]{figure/gen_all/rotX.pdf}&
%         \includegraphics[width=0.3\linewidth]{figure/gen_all/rotY.pdf}&
%         \includegraphics[width=0.3\linewidth]{figure/gen_all/rotZ.pdf}\\
%         (d) Image rotated in \textit{x}-axis ($r_{pitch}$) & (e) Image rotated in \textit{y}-axis ($r_{yaw}$) & (f) Image rotated in \textit{z}-axis ($r_{roll}$) \\
% \end{tabular}
% \vspace{0.1cm}
% \caption{Examples of a original image (a) and generated images (b-f). (a) The red square represents cropped image by the size 244$\times$804.}
% \vspace{-2mm}
% \label{gen_all}
% \end{figure*}



% \subsection{Details of generated datasets}
% \label{exp:datagen}
% %We synthesize the images by changing the roll, pitch, and yaw from $0^{\circ}$ to $5^{\circ}$ by increasing every $1^{\circ}$ for rotation changes. 
% We only synthesize the images by changing the $y$-axis translation for the translation changes. 
% We set left images as reference images and regard right images in KITTI stereo as $x$-axis translated images. 
% Previous and next frames in the time domain can be regarded as $z$-axis translated images. We observe consistent performance whether the vehicle is positioned at the front or at the rear.
% Thus, we conduct the experiments with three rotation changes (roll, pitch, and yaw) and two translation changes ($x$-axis, and $y$-axis) to identify the components that degrade performance as shown in \figref{Qualitative_result_kitti}. 


% Also, we reproduce the same situation as seen in the \figref{Qualitative_result_kitti}, where the car height and pitch(rotation $x$) is different.
% We note that the right, bottom, and frontal moving directions of a car are $x$-, $y$- and $z$-axis, respectively as illustrated in \figref{Qualitative_result_kitti}. 


%\subsection{Quantitative and qualitative results}

% \begin{figure}[t]
% \scriptsize
%     \resizebox{\columnwidth}{!}{
%     \centering
%     \begin{tabular}{c@{\hspace{0.1mm}}c@{\hspace{0.1mm}}}
%         \includegraphics[width=6cm]{figure/2D_results/results_2D_short.pdf} \\(a) Translation changes \\
%         \includegraphics[width=6cm]{figure/2D_results/results_2D_short.pdf}\\
%          (b) Rotation changes\\
%     \end{tabular}
%     }
%     \vspace{-0.1cm}
%     \caption{Quantitative 2D detection results. Performance change($\%$) means the percentage of the moderate 2D performance compared to original moderate 2D performance of each model(MonoGRNet \cite{qin2019monogrnet}, SMOKE \cite{liu2020smoke}, MonoDLE \cite{ma2021delving}, MonoFLEX \cite{zhang2021objects}).}
%     \vspace{-2mm}
% \label{results_2D}
% \end{figure}


%We perform a performance evaluation on all the generated images and identify how the 3D performance of the networks changes for different camera extrinsic parameters. 
\subsection{Comparison to state-of-the-art methods}
\label{sec:state}
We compare our method to state-of-the-art methods, MonoGRNet \cite{qin2019monogrnet}, SMOKE \cite{liu2020smoke}, MonoDLE \cite{ma2021delving}, and MonoFLEX \cite{zhang2021objects}.
All the networks are trained using the cropped original KITTI left images $\mathbf{I}_{ref}$ as shown in \figref{Qualitative_result_kitti}-(a).
The object 3D bounding boxes in \figref{Qualitative_result_kitti} are predicted by passing the various rotated images and translated images $\mathbf{I}_{target}$ generated by following \secref{sec:datageneration} through the trained networks.
We investigate the performance drop of the baseline networks given the images captured at different orientations and positions.
The qualitative results are shown in \figref{Qualitative_result_kitti}-(b-f) and the quantitative results are reported in \figref{3D_results_graph} and \tabref{Part_3D_results}.
We report both $AP_{3D}~(IoU=0.7)$ and $AP_{BEV}$ in \tabref{Part_3D_results}. 
We observe that the $AP_{BEV}$ of conventional methods dropped slightly because it measures the average precision in a 2D Bird-Eye-View projected space. 
All results analysis is conducted based on $AP_{3D}$.
Overall, the translation changes rarely degrade performance in all of the state-of-the-art methods. However, rotation changes, especially in roll and pitch axes, sharply lower the average precision of all competing methods, while the proposed method retains its performance.


\begin{figure*}[t]
    \centering
    \footnotesize
    %\resizebox{\columnwidth}{!}{
    \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}}
         \includegraphics[width=0.2\linewidth]{figure/real_img/before/000551_3D_before.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/after/000551_3D_after.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/before/1.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/after/1.pdf} \\
         \includegraphics[width=0.2\linewidth]{figure/real_img/before/001016_3D_before.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/after/001016_3D_after.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/before/10.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/after/10.pdf} \\
         \includegraphics[width=0.2\linewidth]{figure/real_img/before/4.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/after/4.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/before/5.pdf}&
         \includegraphics[width=0.2\linewidth]{figure/real_img/after/5.pdf} \\
         %\includegraphics[width=0.24\linewidth]{figure/real_img/before/6.pdf}&
         %\includegraphics[width=0.24\linewidth]{figure/real_img/after/6.pdf}&
         %\includegraphics[width=0.24\linewidth]{figure/real_img/before/7.pdf}&
         %\includegraphics[width=0.24\linewidth]{figure/real_img/after/7.pdf} \\
         MonoDLE & Ours & MonoDLE & Ours \\
    \end{tabular}%}
    \vspace{-0.1cm}
    \caption{Qualitative results of the baseline model (MonoDLE \cite{ma2021delving}) and our method on real-world datasets. Training datasets are captured with a passenger car and test datasets are captured with a truck. We visualize the regressed 3D bounding box from MonoDLE and ours.}
    \vspace{-4mm}
\label{real_img}
\end{figure*}

%%% 현재 예시 사진 (python)
\begin{figure}[t]
\scriptsize
    \centering
    \begin{tabular}{c@{\hspace{0.1mm}}} \includegraphics[width=7cm]{figure/monoef/MonoEF.png}\\
    \end{tabular}
    \vspace{-0.1cm}
    \caption{Results comparison of MonoEF \cite{zhou2021monocular} and ours using $AP_{40}~(IoU=0.7)$.}
    \vspace{-0.65cm}
\label{monoef}
\end{figure}

% monoef 와 같이 feature 

\subsubsection{Quantitative/qualitative results from synthetic datasets}
We synthesize the images by changing the roll ($r_{roll}$), pitch ($r_{pitch}$), yaw ($r_{yaw}$), and pitch with $y$-axis translation from $0^{\circ}$ to $5^{\circ}$ by increasing every $1^{\circ}$ for rotation changes. 
We evaluate the performance changes as the degree of rotation increases. 
As shown in \figref{3D_results_graph}, the average precision $AP_{3D}$ of all the methods, MonoGRNet, SMOKE, MonoDLE, and MonoFLEX decreases sharply as the degree of rotation increases on the roll and pitch axes. After $3^{\circ}$ rotation, the conventional methods show around $10\%$ of the original results and reach about $1\%$ with $5^{\circ}$ rotation.
Meanwhile, the proposed module avoids the performance degradation exhibited by all the competitive methods. 
It achieves about $80\%$ of the original results with $3^{\circ}$ rotation and about $60\%$ with $5^{\circ}$ rotation. 
We also observe that the performance from pitch rotated images and that from both pitch rotated and $y$-axis translated images are similar. This means the translation in the $y$-axis rarely results in performance drop.
We report the $AP_{3D}$ performances of all the competitive methods with ours in \tabref{Part_3D_results}. 
Some part of results are included in \figref{3D_results_graph}.
We additionally describe the results of yaw rotation ($r_{yaw}$) and $x$-axis translation.
The results from yaw rotation show that the conventional methods produce around $65\%$ of the original results.
The performance drop ratio is relatively lower than the results from roll or pitch rotation ($r_{pitch}, r_{roll}$) as shown in \figref{3D_results_graph}. 
This is because the monocular 3D object detection model learns the vehicle directly in the yaw axis while the heading directions in the roll and pitch axes have not been trained.
The compensation for object heading direction in the yaw axis does not significantly increase performance. 
The proposed module increases  performance by about $10\%$ of the conventional methods. 
We also visualize the 3D bounding boxes in 3D space in \figref{visualize_3D}.
The results show that our 3D object detection method outperforms the conventional methods not only in 2D projected space but also in real 3D space.
For the translation changes in $x$-axis or $y$-axis, the performance is almost retained, as shown in \tabref{Part_3D_results}.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


%%% PDF로 바꿔야함
\begin{figure}[t!]
\resizebox{\columnwidth}{!}{
    \centering
    % \footnotesize
    \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}}
         \includegraphics[width=0.46\linewidth, height=2cm]{figure/visualize_3D/imgs/000003.pdf}&
         \includegraphics[width=0.46\linewidth, height=2cm]{figure/visualize_3D/000003.pdf}\\
         \includegraphics[width=0.46\linewidth, height=2cm]{figure/visualize_3D/imgs/000016.pdf}&
         \includegraphics[width=0.46\linewidth, height=2cm]{figure/visualize_3D/000016.pdf}\\
         (a) Images with pitch rotation & (b) 3D bounding boxes in 3D \\
    \end{tabular}%
    }
    \caption{Visualization of 3D bounding box in 3D space. We visualize the 3D bounding boxes estimated from ours and the baseline model. Boxes marked in red, green and blue are the ground truth, baseline method, and our method, respectively.}
    \vspace{-0.8cm}
\label{visualize_3D}
\end{figure}



%\subsubsection{Performance w.r.t. Translation changes}
%Translation X, Y
% translation X, Y는 카메라가 상하좌우로 움직이는 것이다. 한 카메라가 상하좌우로 움직이는 것과 같은 효과라 볼 수 있으므로 원래 데이터 대비했을 때 성능이 조금 바뀔 수는 있으나, translation X와 Y에서 existing method와 ours의 성능에 변화가 없다.  
% translation X, Y 는 카메라 상하좌우로 움직이는 것과 같다. 
% As shown in \tabref{Part_3D_results}, degradation 
%Translation X, Y is the movement of the camera up, down, left, and right. As it can be seen as the same effect as the learned camera moving up, down, left and right, the performance is about $80\%$ of the original results and there is no performance difference between the existing method and ours in translation X and Y as shown \tabref{Part_3D_results}. 

% 실제 환경에서는 카메라의 translation Y가 다를 때 field of view를 맞춰주기 위해 pitch를 변화시키는 경우가 많다. 이러한 변칙적인 환경에서는 rotation의 영향을 받아 성능이 떨어진다. pitch의 변화로 인한 성능변화와 같은 이유며, 우리의 방법은 이러한 환경에서도 성능을 높였다.
%Translation Y + pitch
%In a real settings, when the translation Y of the camera is different, the pitch is often changed to match the field of view.
% To reproduce the situation in \figref{overview}, we generate translation Y + Pitch dataset.
% When the translation Y increases by 5cm, the pitch increases by 1 degree.
% As shown in \figref{3D_results_graph} and \tabref{Part_3D_results}, translation Y + Pitch dataset shows a similar tendency to the pitch dataset. The conventional methods show around $10\%$ of original results in $3^{\circ}$ and it reaches under $1\%$ in $5^{\circ}$. Meanwhile, the proposed module protects the performance similar to $r_{pitch}$.
% The performance degradation is larger than when there is only translation, so it seems to be the effect of $r_{pitch}$. Our method improves the performance of the monocular 3D object detection networks as shown \figref{3D_results_graph} and \tabref{Part_3D_results}. 


Lastly, we compare our method to MonoEF \cite{zhou2021monocular}, which mitigates the extrinsic parameter perturbations of the 3D
detection task. 
The method predicts the camera extrinsic with respect to the road plane, then the feature maps of the input image are transferred using the estimated camera extrinsic.
Since the code for MonoEF is not released, we implement the algorithm without the extrinsic estimation part. 
For a fair comparison, we use the GT camera extrinsic and transfer the image features using GT extrinsic parameters.
As shown in \figref{monoef}, the proposed method outperforms the conventional compensation method.
This means the compensation of the 3D bounding box regression is more effective in an output space rather than the feature space. 

\subsubsection{Qualitative results from Real-world datasets}
To show the effectiveness of the proposed method, we conduct qualitative experiments with real-world datasets.
The training datasets are captured using a normal passenger car and the test datasets are captured using a truck. We use the same camera, which means the camera intrinsic is the same. 
The height of the camera of the two vehicles from the road is different.
To set a similar field of road view, the camera in the truck is tilted on the pitch axis.
The camera setting is equivalent to the TransY+Pitch in \figref{3D_results_graph} and \tabref{Part_3D_results}.
We train the baseline model, MonoDLE, with our real-world datasets in a supervised manner. 
We compare the results from the MonoDLE and ours in \figref{real_img}.
Our method does not require an additional training process. We use the MonoDLE model and the proposed compensation module.
The results show that with the existing method the estimated 3D bounding box is misaligned with the ground plane. On the other hand, our method estimates the 3D bounding box to fit the ground plane and the orientation of the object.

\subsection{Analysis of 2D object detection}
2D object detection is a sub-part of conventional 3D object detection networks.
2D detection is utilized as a guideline to regress projected 3D points.
We investigate the 2D detection performance of the networks with respect to the translation and rotation changes.
As shown in \figref{results_2D}, we observe that both translation and rotation changes rarely affect the performance of 2D object detection. 
Even with the $5^{\circ}$ rotated images, the 2D detection performance of the networks does not decrease significantly and is maintained at more than 80\% of the original performance. 

\begin{figure}[t!]
\scriptsize
    \centering
    \begin{tabular}{c@{\hspace{0.1mm}}} \includegraphics[width=9cm]{figure/2D_results/results_2D_short.pdf}\\
    \end{tabular}
    \vspace{-0.1cm}
    \caption{Quantitative results on 2D object detection. Performance change ($\%$) means the percentage of the moderate 2D performance compared to original moderate 2D performance of each model (MonoGRNet \cite{qin2019monogrnet}, SMOKE \cite{liu2020smoke}, MonoDLE \cite{ma2021delving}, MonoFLEX \cite{zhang2021objects}).}
    \vspace{-2mm}
\label{results_2D}
\end{figure}

\subsection{Analysis of individual factors in 3D object detection}
We deeply analyze the individual prediction of 3D object detection networks.
We perform extensive experiments to figure out which of the various factors in the3D bounding box regression is significantly affected by small prediction errors or changes in camera rotation in \tabref{change_gt}. 
We use MonoDLE \cite{ma2021delving} as our baseline model for the ablation studies.
As described in \secref{sec:ours}, MonoDLE independently predicts each of the components, projected 3D points $[x_{2d}, y_{2d}]$, depth $z_{3d}$, yaw angle $r_{yaw}$, Bounding Box (BB) size $\mathbf{S}=[h,w,l]$, then the object 3D bounding box is computed using \eqnref{our_method}.
We measure the performance with $3^{\circ}$ pitch, yaw, roll rotated images, and original images.
We use the prediction values from MonoDLE, but replace the factor with GT values in \tabref{change_gt}-(a-e).
We use all GT values, but replace the factor with prediction values in \tabref{change_gt}-(f-j).
The results from the baseline model in the top row of \tabref{change_gt} demonstrate that the precision from pitch and roll rotated images is significantly degraded while the yaw rotation only slightly reduced performance. 
This means that camera rotations in the pitch and roll axis (not the yaw axis) are dominant factors affecting the drop in 3D object detection performance, just as was observed with \tabref{sec:state}.


\subsubsection{Bounding box size $\mathbf{S}=[h,w,l]$}
\label{sec:bb}
As reported in \tabref{change_gt}-(a), the performance of the baseline model, where the predicted BB size $\mathbf{S}=[h,w,l]$ is replaced by the GT value, marginally improved from 11.3\% to 13.3\%.
This means that the baseline network regresses very accurately on the 3D BB size, and small errors in the 3D BB prediction only slightly affect precision.
Moreover, we observe that the 3D object detection performance from the images rotated in pitch, yaw, and roll axis is also marginally improved (\textit{e.g.} $\text{pitch}_{3}$: 1.76\% to 2.12\%). Even though the GT BB size is utilized, the results with this level of precision are not available to be utilized. 
We can conclude that BB size is not a dominant factor in thedegraded performance at different camera settings.
The results in \tabref{change_gt}-(f), which use all GT values except the predicted BB size, show about $76\%$-$79\%$ $AP_{40}$ even with rotated images.
This is much higher precision than the results from the baseline.
This demonstrates that the 3D object detector accurately regresses BB size despite the rotated image being input.


%%% yaw 3 결과 뽑기
\begin{table}[t!]
\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{lcccc}
\hline
\multicolumn{1}{c|}{replace factors with gt values} & \multicolumn{1}{c|}{original} & \multicolumn{1}{c|}{$pitch_3$} & \multicolumn{1}{c|}{$yaw_3$} & $roll_3$ \\ \hline
\multicolumn{1}{c}{Baseline (MonoDLE)} & \multicolumn{1}{c}{11.3} & \multicolumn{1}{c}{1.76} & 8.61 & 0.99 \\ \hline
(a) with   BB size                            & 13.3                          & 2.12                        & 9.76  & 1.38 \\
(b) with   projected3D                       & 12.0                          & 2.01                        & 9.42   & 1.27\\
(c) with   yaw angle                        & 11.8                          & 1.78                        & 10.5 & 1.31\\ 
(d) with   3D location                       & 77.6                          & 75.4                        & 74.8   & 72.1\\
(e) with   depth                             & 67.0                          & 36.7                        & 58.1  & 12.1\\\hline
(f) without   BB size                            & 78.2                          & 76.1                        & 77.4  & 78.9 \\
(g) without   projected3D                        & 76.4                          & 56.8                        & 74.4 & 18.9\\
(h) without   yaw angle                         & 69.8                          & 68.4                        & 69.4  & 67.1 \\ 
(i) without   3D location                        & 13.5                          & 11.8                        & 12.7 & 12.1 \\
(j) without   depth& 14.2& 12.5& 13.7 & 12.9 \\\hline
\end{tabular}
}
\caption{Performance analysis to investigate the dominant factors affecting the 3D detection performance. We use $AP_{40}~(IoU=0.7)$ under moderate setting on the KITTI validation set for 3D detection performance evaluation. (a)-(e) We replace the predictions to GT values. (f)-(j) We use all GT values and replace GT values to predictions.}
\label{change_gt}
\vspace{-0.4cm}
\end{table}


\subsubsection{Projected 3D object center $[x_{2d}, y_{2d}]$} 
\label{sec:p3d}
Similar to \secref{sec:bb}, we conduct a performance analysis with/without GT projected 3D points $[x_{2d}, y_{2d}]$ in \tabref{change_gt}-(b, g), respectively.
The results show aspects similar to those observed in the BB size analysis.
As reported in \tabref{change_gt}-(b), the performance of the baseline model with GT projected 3D points marginally improved, from 11.3\% to 12.0\%.
This means that the projected 3D points are accurately predicted.
Moreover, we observe that the 3D object detection performance from the images rotated in pitch, yaw, and roll axis is also marginally improved (\textit{e.g.} $\text{pitch}_{3}$: 1.76\% to 2.01\%) although the GT projected 3D points are utilized.
We can conclude that projected 3D points are not a dominant factor in  performance degradation with different camera settings.



% As seen in \tabref{change_gt}-(b), replacing projected 3D object center with ground truth value does not significantly affect the performance. In \figref{Qualitative_result_kitti}, when the camera rotates, there is no problem in the network capturing the projected 3D object center. In \tabref{change_gt}-(g) where all factors except projected 3D object center is replaced with ground truth values, performance increases in all camera settings. However, $r_{pitch}$ and $r_{roll}$ are low performance compared to $r_{yaw}$ and original. Also, there is difference in $r_{pitch}$ and $r_{roll}$. It seems that it is more affected by depth and 3D location in $r_{roll}$.

\subsubsection{Heading direction, yaw angle $r_{yaw}$}
\tabref{change_gt}-(c, h) shows the performance with/without GT heading direction, yaw angle $r_{yaw}$.
These results also show aspects similar to those observed in the analysis of BB size and 3D projected center, as described in \secref{sec:bb} and \secref{sec:p3d}.
The results in \tabref{change_gt}-(c), applied GT yaw angle are almost similar to the results from baseline.
This means the predicted yaw angle is quite accurate to regress 3D bounding boxes.
The precision from yaw rotated image is much higher than that from roll or pitch rotated images (10.5\% vs 1.78\%, 1.31\%).
This means the conventional methods only consider an objects' yaw angle estimation.
The conventional method requires estimating all heading directions of vehicles, roll, pitch, and yaw for better regression.

\subsubsection{3D object center $[X_c,Y_c,Z_c]$ $\&$ depth $z_{3d}$}
\tabref{change_gt}-(d, e) shows the performance of the baseline model where the predicted 3D location $[X_c,Y_c,Z_c]$ or depth $z_{3d}$ is replaced by the GT values.
Surprisingly, all the results in \tabref{change_gt}-(d) including the original, $\text{pitch}_3$, $\text{yaw}_3$, and $\text{roll}_3$ achieve an average precision of over 70\%. 
This means the predictions of BB size and yaw angles are quite accurate while the 3D location prediction is relatively less accurate. 
With better estimates of 3D location, the performance of the 3D object detector will be drastically improved.
Even with the rotated images, the performance is retained. 
Although the 3D heading directions of the roll and pitch rotated cameras have some errors, the accuracy of the 3D positions mitigate the AP3D performance degradation.
In the conventional methods, the 3D object center is computed using the back-projection of the 2D projected center with the depth $z_{3d}$ by following \eqnref{eq:objectcenter}.
We additionally analyze  performance changes with GT depth value in \tabref{change_gt}-(e). 
The overall precision is lower than the results in \tabref{change_gt}-(d), but all results from original and rotated images achieves better performance than the baseline model.
Therefore, the depth and 3D location are the dominant causes of the performance drop. 


==> hdbbmghpkppdgpsxjsjpbxswkydbdxrq/6_conclusion.tex <==
\section{Conclusion}
In this paper, we deeply analyze the factors that lead to performance degradation when pretrained 3D objection models are applied to other camera systems. We found that the camera pose changes, especially the roll and pitch rotation changes, critically affect the performance of the 3D object detection. 
Based on these observations, we propose a generalized 3D object detection method. 
Although the method is trained on just one specific camera setup, it is applicable to various camera systems.
The proposed module is generally applied to the recent monocular 3D object detectors, such as MonoGRNet \cite{qin2019monogrnet}, SMOKE \cite{liu2020smoke}, MonoDLE \cite{ma2021delving}, and MonoFLEX \cite{zhang2021objects}. 
Without any further training, the proposed method provides  about 6-to-10 times improved $AP_{3D}$ compared with state-of-the-art methods. 
%Also, it is expected that by learning through the proposed algorithm using real data in various camera extrinsic settings, we could generate a model that is more robust to various camera extrinsic settings. 
%% limitations: 결국 만든 이미지이기 때문에 다양한 카메라 환경에서 얻은 실제 데이터와는 조금의 차이가 있을 수 있다. 또한, projected 3D object center를 구하지 않는 네트워크에서는 다르게 작용할 수 있다. 우리는 다양한 카메라 환경에서도 robust 하게 더 잘 추정할 수 있고 기존의 데이터에서는 더 추정을 잘 하는 네트워크를 만들 생각이다. 

%우리는 monocular 3d object detection이 학습하지 않은 다른 카메라 데이터 셋에서 ap3d 성능이 많이 떨어지는 것을 실험을 통해 확인했다. ap3d를 구성하는 label들을 바꿔가며(w,h,l, alpha, x, y,z 등) 성능이 떨어지는 주 원인을 규명했고 이를 보완하는 알고리즘을 개발하였다. warping 으로 생성된 데이터를 이용하는 것이 아니라 여러 각도의 실제 데이터를 이용해 제안한 알고리즘을 통해 학습하면 더욱 여러 환경에 강건한 모델을 생성할 수 있을 것으로 예상된다.
% 우리는 다양한 데이터 셋을 만들었고 다른 카메라 환경에서 2D 성능은 하락하지 않은 것을 알았다. 또한 우리 실험은 3D 성능은 다른 카메라 환경에서 하락하는 것을 보여주었다. 우리는 어떠한 카메라 환경에서 성능이 저하되는지 규명하였고 이러한 문제를 해결하는 방법을 제안하였다. 우리의 방법은 기존의 방법에 비해 다양한 카메라 환경에서 성능이 높았다. 제안한 방법을 통해 다양한 카메라 환경에서 새로운 데이터로 학습하는 것

%\section{Acknowledgment}
%This research was supported in part by Autonomous Driving Center, R\&D Division, Hyundai Motor Company.


==> hdbbmghpkppdgpsxjsjpbxswkydbdxrq/def2.tex <==
%
%
%   def.set
%
%       seungjin@postech.ac.kr
%
%       Last updated:
%       September 19, 2004
%
%       A set of my definitions and new commands
%
%


% math bold for lower cases (a-z)
\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bc}{{\mathbf{c}}}
\newcommand{\bd}{{\mathbf{d}}}
\newcommand{\bolde}{{\mathbf{e}}}
\newcommand{\boldf}{{\mathbf{f}}}
\newcommand{\bg}{{\mathbf{g}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\bi}{{\mathbf{i}}}
\newcommand{\bj}{{\mathbf{j}}}
\newcommand{\bk}{{\mathbf{k}}}
\newcommand{\bl}{{\mathbf{l}}}
\newcommand{\bm}{{\mathbf{m}}}
\newcommand{\bn}{{\mathbf{n}}}
\newcommand{\bo}{{\mathbf{o}}}
\newcommand{\bp}{{\mathbf{p}}}
\newcommand{\bq}{{\mathbf{q}}}
\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bt}{{\mathbf{t}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bz}{{\mathbf{z}}}





% math bold for upper cases (A-Z)
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}





% calligraphic
\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}
\newcommand{\calbX}{\mbox{\boldmath $\mathcal{X}$}}
\newcommand{\calbY}{\mbox{\boldmath $\mathcal{Y}$}}


\newcommand{\bcalA}{\mbox{\boldmath $\calA$}}
\newcommand{\bcalB}{\mbox{\boldmath $\calB$}}
\newcommand{\bcalC}{\mbox{\boldmath $\calC$}}
\newcommand{\bcalD}{\mbox{\boldmath $\calD$}}
\newcommand{\bcalE}{\mbox{\boldmath $\calE$}}
\newcommand{\bcalF}{\mbox{\boldmath $\calF$}}
\newcommand{\bcalG}{\mbox{\boldmath $\calG$}}
\newcommand{\bcalH}{\mbox{\boldmath $\calH$}}
\newcommand{\bcalI}{\mbox{\boldmath $\calI$}}
\newcommand{\bcalJ}{\mbox{\boldmath $\calJ$}}
\newcommand{\bcalK}{\mbox{\boldmath $\calK$}}
\newcommand{\bcalL}{\mbox{\boldmath $\calL$}}
\newcommand{\bcalM}{\mbox{\boldmath $\calM$}}
\newcommand{\bcalN}{\mbox{\boldmath $\calN$}}
\newcommand{\bcalO}{\mbox{\boldmath $\calO$}}
\newcommand{\bcalP}{\mbox{\boldmath $\calP$}}
\newcommand{\bcalQ}{\mbox{\boldmath $\calQ$}}
\newcommand{\bcalR}{\mbox{\boldmath $\calR$}}
\newcommand{\bcalS}{\mbox{\boldmath $\calS$}}
\newcommand{\bcalT}{\mbox{\boldmath $\calT$}}
\newcommand{\bcalU}{\mbox{\boldmath $\calU$}}
\newcommand{\bcalV}{\mbox{\boldmath $\calV$}}
\newcommand{\bcalW}{\mbox{\boldmath $\calW$}}
\newcommand{\bcalX}{\mbox{\boldmath $\calX$}}
\newcommand{\bcalY}{\mbox{\boldmath $\calY$}}
\newcommand{\bcalZ}{\mbox{\boldmath $\calZ$}}

\newcommand{\sfA}{\mbox{$\mathsf A$}}
\newcommand{\sfB}{\mbox{$\mathsf B$}}
\newcommand{\sfC}{\mbox{$\mathsf C$}}
\newcommand{\sfD}{\mbox{$\mathsf D$}}
\newcommand{\sfE}{\mbox{$\mathsf E$}}
\newcommand{\sfF}{\mbox{$\mathsf F$}}
\newcommand{\sfG}{\mbox{$\mathsf G$}}
\newcommand{\sfH}{\mbox{$\mathsf H$}}
\newcommand{\sfI}{\mbox{$\mathsf I$}}
\newcommand{\sfJ}{\mbox{$\mathsf J$}}
\newcommand{\sfK}{\mbox{$\mathsf K$}}
\newcommand{\sfL}{\mbox{$\mathsf L$}}
\newcommand{\sfM}{\mbox{$\mathsf M$}}
\newcommand{\sfN}{\mbox{$\mathsf N$}}
\newcommand{\sfO}{\mbox{$\mathsf O$}}
\newcommand{\sfP}{\mbox{$\mathsf P$}}
\newcommand{\sfQ}{\mbox{$\mathsf Q$}}
\newcommand{\sfR}{\mbox{$\mathsf R$}}
\newcommand{\sfS}{\mbox{$\mathsf S$}}
\newcommand{\sfT}{\mbox{$\mathsf T$}}
\newcommand{\sfU}{\mbox{$\mathsf U$}}
\newcommand{\sfV}{\mbox{$\mathsf V$}}
\newcommand{\sfW}{\mbox{$\mathsf W$}}
\newcommand{\sfX}{\mbox{$\mathsf X$}}
\newcommand{\sfY}{\mbox{$\mathsf Y$}}
\newcommand{\sfZ}{\mbox{$\mathsf Z$}}





% math bold for lower cases (Greek letters)
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bdelta}{\mbox{\boldmath $\delta$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bvarepsilon}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\boldeta}{\mbox{\boldmath $\eta$}}
\newcommand{\btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bvartheta}{\mbox{\boldmath $\vartheta$}}
\newcommand{\biota}{\mbox{\boldmath $\iota$}}
\newcommand{\bkappa}{\mbox{\boldmath $\kappa$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bnu}{\mbox{\boldmath $\nu$}}
\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bpi}{\mbox{\boldmath $\pi$}}
\newcommand{\bvarpi}{\mbox{\boldmath $\varpi$}}
\newcommand{\brho}{\mbox{\boldmath $\rho$}}
\newcommand{\bvarrho}{\mbox{\boldmath $\varrho$}}
\newcommand{\bsigma}{\mbox{\boldmath $\sigma$}}
\newcommand{\bvarsigma}{\mbox{\boldmath $\varsigma$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\bupsilon}{\mbox{\boldmath $\upsilon$}}
\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bvarphi}{\mbox{\boldmath $\varphi$}}
\newcommand{\bchi}{\mbox{\boldmath $\chi$}}
\newcommand{\bpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\bomega}{\mbox{\boldmath $\omega$}}





% math bold for upper cases (Greek Letters)
\newcommand{\bGamma}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bDelta}{\mbox{\boldmath $\Delta$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\bLambda}{\mbox{\boldmath $\Lambda$}}
\newcommand{\bXi}{\mbox{\boldmath $\Xi$}}
\newcommand{\bPi}{\mbox{\boldmath $\Pi$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bUpsilon}{\mbox{\boldmath $\Upsilon$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bPsi}{\mbox{\boldmath $\Psi$}}
\newcommand{\bOmega}{\mbox{\boldmath $\Omega$}}





% vector notation for lower cases (a-z)
\newcommand{\veca}{{\vec{\ba}}}
\newcommand{\vecb}{{\vec{\bb}}}
\newcommand{\vecc}{{\vec{\bc}}}
\newcommand{\vecd}{{\vec{\bd}}}
\newcommand{\vece}{{\vec{\bolde}}}
\newcommand{\vecf}{{\vec{\boldf}}}
\newcommand{\vecg}{{\vec{\bg}}}
\newcommand{\vech}{{\vec{\bh}}}
\newcommand{\veci}{{\vec{\bi}}}
\newcommand{\vecj}{{\vec{\bj}}}
\newcommand{\veck}{{\vec{\bk}}}
\newcommand{\vecl}{{\vec{\bl}}}
\newcommand{\vecm}{{\vec{\bm}}}
\newcommand{\vecn}{{\vec{\bn}}}
\newcommand{\veco}{{\vec{\bo}}}
\newcommand{\vecp}{{\vec{\bp}}}
\newcommand{\vecq}{{\vec{\bq}}}
\newcommand{\vecr}{{\vec{\br}}}
\newcommand{\vecs}{{\vec{\bs}}}
\newcommand{\vect}{{\vec{\bt}}}
\newcommand{\vecu}{{\vec{\bu}}}
\newcommand{\vecv}{{\vec{\bv}}}
\newcommand{\vecw}{{\vec{\bw}}}
\newcommand{\vecx}{{\vec{\bx}}}
\newcommand{\vecy}{{\vec{\by}}}
\newcommand{\vecz}{{\vec{\bz}}}

\newcommand{\vecxi}{{\vec{\bxi}}}
\newcommand{\vecphi}{{\vec{\bphi}}}
\newcommand{\vecvarphi}{{\vec{\bvarphi}}}
\newcommand{\vecbeta}{{\vec{\bbeta}}}
\newcommand{\vecdelta}{{\vec{\bdelta}}}
\newcommand{\vectheta}{{\vec{\btheta}}}


% set of numbers
\newcommand{\Real}{\mathbb R}
\newcommand{\Complex}{\mathbb C}
\newcommand{\Natural}{\mathbb N}
\newcommand{\Integer}{\mathbb Z}


% color
%\definecolor{orange}{rgb}{1,0.3,0}
%\definecolor{copper}{rgb}{1,.62,.40}


% ets
\newcommand{\bone}{\mbox{\boldmath $1$}}
\newcommand{\bzero}{\mbox{\boldmath $0$}}
\newcommand{\0}{{\bf 0}}

\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\bee}{\begin{eqnarray*}}
\newcommand{\eee}{\end{eqnarray*}}

\newcommand{\matrixb}{\left[ \begin{array}}
\newcommand{\matrixe}{\end{array} \right]}   

\newtheorem{theorem}{{Theorem}}
\newtheorem{lemma}{{Lemma}}
\newtheorem{corollary}{{Corollary}}
\newtheorem{definition}{{Definition}}
\newtheorem{proposition}{{Proposition}}
\newtheorem{remark}{{Remark}}
\newtheorem{example}{{Example}}
%\newtheorem{algorithm}{{Algorithm}}

\newcommand{\argmax}{\operatornamewithlimits{\arg \max}}
\newcommand{\argmin}{\operatornamewithlimits{\arg \min}}

\newcommand{\mean}[1]{\left \langle #1 \right \rangle}
\newcommand{\ave}{\mathbb E}
\newcommand{\E}{\mathbb E}
\newcommand{\empha}[1]{{\color{red} \bf #1}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\incomplete}[1]{\textcolor{red}{#1}}



\def\doublespace{\renewcommand{\baselinestretch}{2}\large\normalsize}
\def\singlespace{\renewcommand{\baselinestretch}{1}\large\normalsize}
\def\onehalfspace{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\def\onequaterspace{\renewcommand{\baselinestretch}{1.3}\large\normalsize}
\def\threequaterspace{\renewcommand{\baselinestretch}{1.7}\large\normalsize}
\def\smallspace{\renewcommand{\baselinestretch}{-.9}\large\normalsize}
\def\tinyspace{\renewcommand{\baselinestretch}{-.7}\large\normalsize}

\newcommand{\tr} { \textrm{tr} }
\newcommand{\re} { \textrm{re} }
\newcommand{\diag} { \textrm{diag} }
\newcommand{\ddiag} { \textrm{ddiag} }
\newcommand{\off} { \textrm{off} }
\newcommand{\vectxt} { \textrm{vec} }

\newcommand{\lla}{\left\langle}
\newcommand{\rra}{\right\rangle}
\newcommand{\llbr}{\left\lbrack}
\newcommand{\rrbr}{\right\rbrack}
\newcommand{\llb}{\left\lbrace}
\newcommand{\rrb}{\right\rbrace}

